Analytical Derivation of Outage Correlation in Random Media Access with Application to Average Consensus in Wireless Networks: Extended Paper Version

We study a finite and fixed relative formation of possibly mobile wireless networked nodes. The nodes apply average consensus to agree on a common value like the formation's center. %Performance of consensus in terms of convergence speed is affected by message losses due path loss and interference. We assume framed slotted ALOHA based broadcast communication. Our work has two contributions. First, we analyze outage correlation of random media access in wireless networks under Nakagami fading. Second, the correlation terms are applied to the so called L2-joint spectral and numerical radii to analyze convergence speed of average consensus under wireless broadcast communication. This yields a unified framework for studying joint optimization of control and network parameters for consensus subject to message losses in wireless communications. Exemplary we show in this work how far outage correlation in wireless broadcast communication positively affects convergence speed of average consensus compared to consensus in the uncorrelated case.

==> 990_intro_alt.tex <==
\begin{abstract}
ADD STUFF

\begin{itemize}
	\item As the average consensus protocol is linear it 
	\item Closed from expressions for slotted ALOHA, general case and Nakagami fading
\end{itemize}



\begin{IEEEkeywords}
L2 joint spectral radius, L2 joint numerical radius, First Order Consensus, Nakagami fading, convergence speed.
\end{IEEEkeywords}

\end{abstract}

\begin{td}
	\begin{itemize}
		\item Voll-Duplex Modell ist gut, um Konsens-Effekte auch fuer kleine Knotenzahlen studieren zu koennen
		\item $ \leadsto \E Y_{ij}Y_{kl}$ berichtigen
		\item 

	\end{itemize}<++>
\end{td}<++>


\textbf{Timetable:}\\
\textbf{By Monday, Feb 3:}
\begin{itemize}
    \item Thorough differentiation from the Haenggi correlation model used in the PPP.
    \item Related work on Nakagami-Fading and outage proabilities in finite networks  $\checkmark$
    \item Proofs of the correlation statements $\checkmark$
    \item Clean and complete statements of the Correlation Proposition and the connection with the ICCCN paper.
    
    
\end{itemize}

\textbf{ By Monday, Feb 10:}
\begin{itemize}
    \item Finalize the Introduction and Related Work according to status quo
    \item General communication focus without particularizing to consensus: 
    \begin{itemize}
        \item Discuss the Simulation/Sampling of the correlation in comparison to the exact formula. 
        \item Provide relative errors in an overview for $n \le 20$ nodes, e.g. n= 6, 10, 15, 20.
        \item Discuss tendencies and possible effects that might have to be considered when using the simulation as an approximation of the formula for $n > 20$ nodes.
    
    
    \end{itemize}
    
    \item Consensus:
        \begin{itemize}
            \item Description of the consensus plots for at least one node deployment for few plausible choices of slots.
            \item Optional: discuss the n=30 case
    \end{itemize}
    
\end{itemize}

    
    
    

\begin{td}
	\item add item Add Lyapunow exponent
\end{td}


\begin{itemize}
	\item Related work: What are the problems/benefits of $r_2,$ versus the lyaponow exp.
	\item Related work: rare events
	\item Related work: Fading!!
	\item Related work: Correlation!!
\end{itemize}


\section{Introduction}
Blabla

%The general direction of research aimed by this work is to quantify the influence of correlations due to media access control schemes on distributed average consensus in a wireless scenario. 
The goal of this work is to quantify the correlations due to media access control schemes for wireless sensor nets (WSN) and for snapshots of ad-hoc-Networks. The results of this work can
be immediately applied to the analysis of distributed cooperative control protocols, such as probabilitstic average consensus \addRef.
Example applications consist of weather measurements (WSN) \addRef and formation control (cooperative control) \addRef.



Concrete, we consider a deployment of $n$ nodes moving in the plane which perform first order, probabilistic average consensus \addRef. As quality measure we use a probabilistic entity describing the instantaneous\footnote{Instantaneous means here that in the analysis we consider snapshots of the nodes' positions. However, the performance of trajectories can be bounded stepwise, e.g. by the measure $\n{\tilde R}$ of \cite{ICCCN19} which is closely related to $r_2.$} exponential decay of the mean squared error/disagreement: the $L^2$-joint spectral radius \addRef or generalized joint spectral radius , which we call $r_2$ \addRef. Since we aim at formal treatment, we employ slotted ALOHA as simple media access scheme for broadcast communication\addRef. Here we have also additional consequences in mind which regard the IEEE 802.11p protocol since the latter can behave like slotted ALOHA at high densities \cite{Baccelli13}. 

The central question of this paper is how the correlation due to each node's choice of the transmission window affects the consensus performance in terms of $r_2,$ compared to a model where packet reception along each link is mutually independent. We have investigated the latter situation in our earlier work \cite{ICCCN19} where we incorporated the SINR physical layer model - recommended in \cite{Iyer09} - with Rayleigh fading and established closed form expressions for successful transmission for each link. In this work we will generalize to Nakagami fading and derive closed form expressions for the covariance between links. These expressions are then fed into the matrix $R$ which is related to $r_2$ by $r_2 = \varrho(R)$ \cite{ICCCN19}, where $\varrho(\cdot)$ denotes the spectral radius of a matrix. 

A second aspect arises when acutally verifying the theorerial findings by simulations of the consensus scenarios.  As we have briefly observed in \cite{ACC18}, rare events of ``bad behavior'' may have large impact on $r_2$ since it is a mean square measure. 
%It would of course be ideal to additionally consider the $L^{1}$-joint spectral radius \addRef characterizing the mean disagreement/error, since it assigns a smaller weight to badly behaving rare events. 
In general, the $L^p$-joint spectral radius (in short $r_p$), $p\ge 1$, characterizes exponential stabiltiy in terms of the mean of the disagreement raised to the $p$-th power ($p$-th mean stability) \addRef{Ogura14}.
Thus, it would of course be ideal to additionally consider $r_1$ \addRef, since it assigns a smaller weight to badly behaving rare events. However, $r_p$ can be computed easily only if $p$ is either even or the random measures representing the communication satisfy a certain geometric property on convex cones \addRef{Protasov} which is not the case for $r_1$ since it would then simply coincide with the essential spectral radius \addRef{Ogura14 oder LA}.

Moreover, a computation of $r_1$ cannot constitute a full solution since the impact of rare events is already present for first mean stability, which is considered in \cite{Moura13}. There, these events are worst case paths with sub-exponential decay in disagreement and are called \textit{large deviations} stemming from the Large Deviation Theory, e.g.\addRef. The authors found that sub-exponential paths do not exist if the communication graph is connected at all instances. The latter is, however, not the case in our modelling scenario. Thus, empirical measurements of the squared disagreement cannot solely be trusted as they can suggest faster convergence than there actually is - a fact that we observe in our simulations for mean square convergence. \comment{Vergleich Bernoulli Simulation, was ist besser?}

%The question comes up why this is the case. To investigate 
To investigate why this is the case 
\begin{itemize}
	\item 2-fold: Im statischen Fall tritt es schon auf \dots
\end{itemize}

It sheds some light on the fact

\begin{itemize}
	\item ICCCN-Paper stellt $k$-Schritt-Abschätzungen bereit.
\end{itemize}


 and investigate 
\textbf{Outline}
\begin{itemize}
	\item iid fading channels
	\item still correlation in slotted aloha $[RW]$
	\item static node setting, no PPP
	\item based on our work \cite{ICCCN19}

	\item SINR \textbf{Further, we feel that an SINR-based model is the minimum level of detail that should be employed to model wireless channel interference} \cite{Iyer09}

\end{itemize}  


==> 9999_aussortiert.tex <==
\subsection{Sketch of Proposition XYZ's proof}

\qed
% END OF PROOF 2
\newpage

\subsection{Slotted CSMA and slot picking ALOHA}
Here, we briefly recapitulate the abstraction of the IEEE 802.11p protocol introduced in \cite{Baccelli13} called slotted CSMA and the corresponding slotted ALOHA model we term slot picking.

Assume a broadcast scenario where all nodes have to transmit a packet every $\tau$ ms. This beacon time interval is called a \df{frame} which is divided into $K$ slots. A node may come with a fixed (time) offset $m = 0, \dots, K-1,$
thus always transmitting 

making it a node of class $m,$ Moreover, each slot is divided into an interframe space and a number $CW$ of subsequent backoff slots followed by the packet transmission duration. 

The beacon time interval is divided into $m$ slots of equal length and the network is dominated by nodes whose \df{backoff counter} is $0$ in the beginning of a slot, i.e. it will send immediately after IFS.


\subsection{Removed}
Motivation: Usual first order continuous time dynamics consensus prototocol with time varying Laplacian $L = L(t)$:
    $$\dot x  = - L x $$
After differentiation, we have
    $$\ddot x = - L \dot x - \dot L x $$
To reduce the blow-up events, let us introduce a velocity dependent damping term with parameter $\sigma:$
$$\ddot x = - L \dot x - \dot L x - \sigma \dot x,$$
or
%$$\ddot x = - (L + \sigma I) \dot x - \frac{\mbox{d}}{\mbox {d} t} (L + I) x  = - \frac{\mbox{d} }{\mbox{d}t}(L + I) x$$
$$\ddot x = - \frac{\mbox{d} }{\mbox{d}t}(L + I) x.$$
After integration (and neglecting the integration constant) we arrive at
$$\dot x = - L^{\sigma}x := -(L + \sigma I) x$$
which translates to the following disagreement dynamics:
    $$\dot \delta = - (L + \sigma \Pi) \delta.$$
Letting $P^\sigma = I - \varepsilon L^\sigma, \varepsilon> 0,$ we have 
	$$ P^\sigma \one = (1-\varepsilon \sigma) \one $$
and 
	$$ P^\sigma $$

When discretizing just substitute L with (L + sigma * id). Thats it. (I know that this does not preserve the average and that 1 is no right-eigenvalue of 1|, this can be fixed e.g. by using sigma * Projection-matrix instead of sigma* id which again has the disadvantage of not having a distributed implementation, but I merely need this as a theoretical construct for analysis and as argument to support the measurements).

I know that having a damping is quite usual in double-integrator systems, e.g. eq (7) [2.pdf].

\subsection{Removed}
 \begin{prp}[\cite{ICCCN19}]
\label{prp:ICCCNprobabilites}
The probability for successful transmission from node $u_i$ to node $u_j,$ while all nodes are constantly competing for slots, is given by the formula
%$$\begin{aligned}p_{ij}(k) &= (1-\frac{1}{k}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{k (\theta + \mu_{mj} / \mu_{ij}})\right)\\
%	&=\frac{k-1}{k^{n-1}} \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(k- \frac{\theta}{\theta + \mu_{mj} / \mu_{ij}}\right)\\ &=: \sum_{m=0}^{n-1}a_{ijm}k^{-m} \end{aligned}$$
%\begin{equation}\label{eqn:p_ij}p_{ij}(m) &= (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{m (\theta + \mu_{mj} / \mu_{ij})}}\right).\end{equation}
\begin{equation}\label{eqn:p_ij}p_{ij}(m) = (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{k\ne i,j} \left(1- \frac{\theta}{m (\theta + \mu_{kj} / \mu_{ij})}\right).\end{equation}
\end{prp} 


 \begin{itemize}
	\item If $L$ is not symmetric, we do not even have $\E x_{\infty} = \frac{1}{n} \one x_0.$
	\item Performance measures: $r2$, Lyapunov exponent
	\item In $r_2$ large, unlikely deviations contribute a lot. $r_1$ cannot be evaluated easily.
	\item Related work criterium in terms of $n$ and $?$: When is $r_2^k$ close to $\E \n{\Pi P_k \dots P_1}^2?$
	\item They say that one should use the $r_2$ if $n \gg 1$ and otherwise the Lyapunov exponent \comment{verify}.
	\item Other related work: symmetric instances, they measure rare subexponential paths. \cite{Moura13}
	\item However, we think neglecting these catastrophic events, which lead to the deviation of the actual squared disagreement from the expected squared disagreement, is not always the best. 
	      Because of the linear nature of the consensus protocol, agents will in practice not be able to follow the protocol once the physical limitations are reached. In simulations one
 	      can model this behavior for instance by simply adding a maximum velocity and thus a maximum possible displacement per time step. If the disagreement is small, bounding the displacement
	      has no effect. If it is large, the displacement will capped. This protocol is, however, no longer linear. To add 
\end{itemize} 


 \textbf{Timetable:}\\
\textbf{By Monday, Feb 3:}
\begin{itemize}
    \item Thorough differentiation from the Haenggi correlation model used in the PPP.
    \item Related work on Nakagami-Fading and outage proabilities in finite networks  $\checkmark$
    \item Proofs of the correlation statements $\checkmark$
    \item Clean and complete statements of the Correlation Proposition and the connection with the ICCCN paper.
    
    
\end{itemize}

\textbf{ By Monday, Feb 10:}
\begin{itemize}
    \item Finalize the Introduction and Related Work according to status quo
    \item General communication focus without particularizing to consensus: 
    \begin{itemize}
        \item Discuss the Simulation/Sampling of the correlation in comparison to the exact formula. 
        \item Provide relative errors in an overview for $n \le 20$ nodes, e.g. n= 6, 10, 15, 20.
        \item Discuss tendencies and possible effects that might have to be considered when using the simulation as an approximation of the formula for $n > 20$ nodes.
    
    
    \end{itemize}
    
    \item Consensus:
        \begin{itemize}
            \item Description of the consensus plots for at least one node deployment for few plausible choices of slots.
            \item Optional: discuss the n=30 case
    \end{itemize}
    
\end{itemize}

    
\subsection{Aussortiert}
  \begin{itemize}
	\item Managing Interference Correlation Through Random Medium Access \cite{Haenggi14}: Correlation between different slots (we consider all of them as a whole) and PPP, ALOHA and FHMA
	\item Hanggi: Correlation between different receivers in PPP, we: correlation between all links in a fixed scenario 
	
	\item still correlation in slotted aloha $[RW]$
	\item Consensus algorithms over fading channels \cite{Chan10}: Fading is not fast fading; just complex circularly symmetric noise with zero mean and variance $1.$ (And: Example graph for slotted ALOHA: convergence time over transmission probability.)
	\item stochastic geometry, interference, non-slotted ALOHA  \cite{Muhle14}
	\item Convergence Speed of the Consensus Algorithm With Interference and Sparse Long-Range Connectivity

\end{itemize} 
\begin{itemize}
	\item Frage: Wie haengen bei uns Kovarianz und Korrelation zusammen
	\item 
\end{itemize}

\begin{itemize}
%	\item Correlation, \cite{Haenggi14}, \cite{Benef04} \comment{(sehr aehnlicher Titel!!)}
	\item 
	\item Consensus \cite{Silva11}, \cite{Fagnani08},  \cite{ICCCN19}, %\cite{Moura13},

	%\item Convergence measures 
\end{itemize}


\begin{itemize}
	\item convergence speed in deterministic average consensus is directly linked to the algebraic connectivity which makes it an ideal prototye application
\end{itemize}
\begin{itemize}
	\item iid fading channels
	\item static node setting, no PPP
	\item SINR \textbf{Further, we feel that an SINR-based model is the minimum level of detail that should be employed to model wireless channel interference} \cite{Iyer09}
\end{itemize}  

\textbf{How is the paper organized?!}   

\begin{td}
	\begin{itemize}
		\item $ \leadsto \E Y_{ij}Y_{kl}$ berichtigen
		\item Mean-square Analyse weit verbreitet. Allerdings schrecken bei $r2$ alle vor den großen Systemen zurück.

	\end{itemize}
\end{td}
 \section{Intro}
 \section{Introduction}
During the past decades wireless sensor networks (WSN) and distributed multiagent systems have attained a lot of research interest in both communication and control community.
The goal of this work is to quantify the outage correlations due to media access control schemes for finite wireless sensor nets (WSN) and for snapshots of multi agent systems. %The results of this work can be immediately applied to the analysis of distributed cooperative control protocols, such as probabilitstic average consensus \addRef{}.
%Example applications consist of weather measurements (WSN) \addRef{} and formation control (cooperative control) \addRef{}.
 
While there is much work on the specifics of either side, few analytical papers consider a unifying approach where the impact of real network phenomenons is measured  directly in terms of distributed control performance as is done in our application.  
The effect of channel correlation has been investigated from a information theoretical point of view \cite{Benef04} as well as average over stochastic point processes \addRef{}. The effect of narrow band fast fading is considered mostly in a point process setting (\comment{belegen}) except for instance in \cite{Nakagami12} which we build upon. 

\addRef{PIMRC18: A pair of closely spaced receivers will receive similar interference even if the interference is received over fading channels that are decorrelated in space and time. This is because the loca- tion of interferers are a common source of randomness, even if the fading channels that they are observed over are not common. \\To the best of our knowledge, this paper is the first attempt to capture both finite network effects and interference correlation within a single unified analysis} 

On the other hand, when consensus is studied from the control perspective,
\addRef{Multi-agent Formation Control with Maintaining and Controlling Network Connectivity und das mit der konvexen Laplacematrix; oversimplified}

Although correlation is beneficial for MIMO capacity\cite{Benef04}, it is often considered bad in media access control (MAC), e.g. (temporal) correlation in different slots has negative impact on retransmissions \cite{Ganti2009}. We analyze outage correlation in the slotted ALOHA media access protocol and measure the effects on distributed schemes in terms of the performance of the average consensus protocol where we observe a benefitial impact for the most part. The applications we have in mind all require broadcast transmission such that Request To Send/Clear To Send (RTS/CTS) mechanisms cannot be applied. With increasing node density also carrier sensing becomes less and less beneficial, e.g. the IEEE 802.11p protocol can behave like slotted ALOHA\cite{Baccelli13}. 

Finally, the simplicity of slotted ALOHA allows for exact theoretical analysis (previous work considers mosty PPP theory \cite{Haenggi14}, \cite{Kim2019}, \cite{Talarico2018}).
Example applications consist of formation control, flocking (cf. the references in \cite{Olfati-Saber2004} and \addRef{ControlPaper}) or purely computational tasks like Gram-Schmidt orthogonalization which can be used to determine the network size \cite{Sluciak2013} or for further signal processing tasks, e.g. \cite{Sluciak2016}.
We make the observation that correlation is beneficial here compare to an (uncorrelated) Bernoulli process with the same (inhomogenous) outage probabilities.

We observe further that the outage correlation consists of two different components, a strong, positively correlated one and a weak, negatively correlated one (Fig. \ref{fig:correlation}??). The strong one shows up between a sender and all recipients and decreases as spatial distance gets bigger. The weak one affects the remaining links.

As application we consider a deployment of $n$ nodes moving in the plane which perform first order, probabilistic average consensus \cite{Olfati-Saber2004}, \cite{Fagnani08}, \cite{Silva11}. As quality measure we use a probabilistic entity describing the instantaneous\footnote{Instantaneous means here that in the analysis we consider snapshots of the nodes' positions.} %However, the performance of trajectories can be bounded stepwise, e.g. by the measure $\n{\tilde R}$ of \cite{ICCCN19} which is closely related to $r_2.$}
exponential decay of the mean squared error/disagreement: the $L^2$-joint spectral radius \cite{Ogura2013} or generalized joint spectral radius, which we call $r_2$ and which allows for exact characterization of (exponential) mean square stability.
Since we aim at formal treatment, we employ a slotted ALOHA variant as simple media access scheme for broadcast communication\addRef{}. %Here we have also additional consequences in mind which regard the IEEE 802.11p protocol since the latter can behave like slotted ALOHA at high densities \cite{Baccelli13}. 

This paper provides the methods to judge how the correlation due to each node's choice of the transmission slot affects the consensus performance in terms of $r_2,$ compared to a model where packet reception along each link is mutually independent. We have investigated the latter situation in our earlier work \cite{ICCCN19} where we incorporated the SINR physical layer model with Rayleigh fading and established closed form expressions for successful transmission for each link. In this work we will generalize to Nakagami fading and derive closed form expressions for the covariance between links. Also we adapt the stepwise bound $w_2$ of \cite{ICCCN19} to the correlated setting. 

An Application to consensus already shows examples of ``correlation network effects.'' For instance, we have found a situation such that when - loosly speakeing - varying the two parameters discrete gain and Nakagami shape parameter, the (sub-)gradient is by trend mirrored at the gain axis when switching from correlated to uncorrelated model.

In the following two sections we discuss related work, the overall notation, and the background needed to discuss the physical layer model. In section \ref{sec:corr} we introduce our MAC layer abstraction for slotted ALOHA and derive expectation and covariance of successful transmissions along links. Section \ref{sec:application} deals with an application of our result to a control theoretic multi agent system performing average consensus. Finally, the conclusion summarizes the paper and points out ideas for future work.

%We provide covariances for two modes \comment{Da fliegt full-duplex wohl raus}: Full and half-duplex. In full duplex we allow sending nodes to receive, while in half-duplex we do not. The former is not realistic. However, 
%since for larger node numbers the two modes approach each other, it can be very interesting to study distributed control in toy examples with reduced complexity, e.g. only 4 nodes with 2 slots which ``behave'' like the case for large node numbers $n$ and $\lfloor{n/2}\rfloor$ slots. \comment{OK, das ist fraglich}



%The general direction of research aimed by this work is to quantify the influence of correlations due to media access control schemes on distributed average consensus in a wireless scenario. 









%A second aspect arises when acutally verifying the theorerial findings by simulations of the consensus scenarios.  As we have briefly observed in \cite{ACC18}, rare events of ``bad behavior'' may have large impact on $r_2$ since it is a mean square measure. 
%In general, the $L^p$-joint spectral radius (in short $r_p$), $p\ge 1$, characterizes exponential stabiltiy in terms of the mean of the disagreement raised to the $p$-th power ($p$-th mean stability) \addRef{Ogura14}.
%Thus, it would of course be ideal to additionally consider $r_1$ \addRef{}, since it assigns a smaller weight to badly behaving rare events. However, $r_p$ can be computed easily only if $p$ is either even or the random measures representing the communication satisfy a certain geometric property on convex cones \addRef{Protasov} which is not the case for $r_1$ since it would then simply coincide with the essential spectral radius \addRef{Ogura14 oder LA}.

%Moreover, a computation of $r_1$ cannot constitute a full solution since the impact of rare events is already present for first mean stability, which is considered in \cite{Moura13}. There, these events are worst case paths with sub-exponential decay in disagreement and are called \textit{large deviations} stemming from the Large Deviation Theory, e.g.\addRef. The authors found that sub-exponential paths do not exist if the communication graph is connected at all instances. The latter is, however, not the case in our modelling scenario. Thus, empirical measurements of the squared disagreement cannot solely be trusted as they can suggest faster convergence than there actually is - a fact that we observe in our simulations for mean square convergence. \comment{Vergleich Bernoulli Simulation, was ist besser?}

%The question comes up why this is the case. To investigate 
%To investigate why this is the case 
%\begin{itemize}
%	\item 2-fold: Im statischen Fall tritt es schon auf \dots
%\end{itemize}

%It sheds some light on the fact
%\begin{itemize}
%	\item ICCCN-Paper stellt $k$-Schritt-Abschätzungen bereit.
%\end{itemize}
 %and investigate 
%\textbf{Outline}

\section{Related work}

The main impact on correlated packet success or - expressed in negative terms - outage correlation - in our work is due to the random set of active nodes within a slot. This kind of correlation is investigated in terms of interference in \cite{Haenggi14}
in point process settings, not for concrete deployments.
Further, it is 

In \cite{Haenggi14} intereference correlation is classified into three different types for each of which further references are provided: 1) Correlation between different time slots of a frame. We consider this type of correlation implicitly since we consider correlation of packet success between different links for the frame as a whole. 2) Correlation between different receive antennas. We consider only one antenna. 3) Correlation between different receivers: This is related to the strong component we observe between links of a common sender and different receivers.

Spatial correlation is mentioned in \addRef{}. We also observe it along the strong component.

In \cite{Ganti2009} spatial and temporal correlation of the interference in ALOHA Ad Hoc Networks is analyzed with point process methods. In contrast, we provide expressions for 
the correlation of the packet success between different links of a fixed deployment.

Correlation in communication channels can have a positive effect in communication systems. In particular for acklowledgements in broadcast communication, (little) empirical study \cite{Alam2012} (two flooding protocols are considered, one with network coding only, one with both, network coding and exploited link correlation).
Correlation of fading in MIMO systems can improve channel capacity \cite{Benef04}. In this work we broadcast study channels without acklowledgements and fading correlation. Communication channels are typically located such that they are not spatially correlated. In such systems correlation is however still present in form interference correlation due to media access. This was for example recently studied in \cite{Haenggi14} where analytical expressions on local delay and jitter \comment{weiter\dots}.
Our analytical derivations significantly differ from that work. Here we are specifically interested in the impact of interference correlation on convergence speed of average consensus using broadcast communication.

The work \cite{Kim2019} is also set in a point process setting. The authors investigate correlation to improve prediction of the packet delivery probabiltiy (PDP). Instead of computing the correlations exactly the authors approximate the correlations.

Recently, outage correlation has been investigaged in a finite point process setting (Binomial, Poisson and Thomas processes) under Rayleigh Fading \cite{Talarico2018}. Although the authors allow for (slotted) ALOHA with call occurance probability, they are mainly concerend with the spatial correlation and the effects of the spatial differences generated by the three point processes; concrete node deployments are not considered.

In\cite{Chan10}, consensus has been considered under fast fading where correlated outages (mainly due to fading) are mentioned without being quantified. In \cite{Kar2009}, \cite{Silva11} abstract correlations can be handled in the consensus framework, however neither a physical model nor a media access model is provided. Also the mean square disagreement measures used there are upper bounds only. In our work we use a different upper bound, $w_2$, \cite{ICCCN19} very well matching the shape of the exact asymptotic bound $r_2$. Both bounds together quite precisely render the outage correlation in terms of (discrete) control gain, fading parameter and number of slots utilized.
An early work meantioning the exactness of $r_2$ but rather analyzing an upper bound for the sake of simplicity is \cite{Boyd2006}.




==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/10_intro.tex <==
\begin{abstract}
%ASTUFF\\[3cm]
We study a finite and fixed relative formation of possibly mobile wireless networked nodes. The nodes apply average consensus to agree on a common value like the formation's center. %Performance of consensus in terms of convergence speed is affected by message losses due path loss and interference.
We assume framed slotted ALOHA based broadcast communication. Our work has two contributions. First, we analyze outage correlation of random media access in wireless networks under Nakagami fading. Second, the correlation terms are applied to the so called L2-joint spectral and numerical radii to analyze convergence speed of average consensus under wireless broadcast communication. This yields a unified framework for studying joint optimization of control and network parameters for consensus subject to message losses in wireless communications. Exemplary we show in this work how far outage correlation in wireless broadcast communication positively affects convergence speed of average consensus compared to consensus in the uncorrelated case.

\begin{IEEEkeywords}
%Outage correlation, spatial correlation, Nakagami fading, average consensus, L2 joint spectral radius, wireless networks, finite networks, convergence speed, half duplex, full duplex, slotted ALOHA, numerical radius, broadcast.
Outage correlation, Nakagami fading, average consensus, L2 joint spectral radius, 
numerical radius, 
wireless networks, slotted ALOHA, broadcast.
\end{IEEEkeywords}
\end{abstract}
\section{Introduction}
During the past decades wireless sensor networks (WSN) and distributed multiagent systems have gained a lot of attention among both communication and control community.
While there is much work on the specifics of either side, only few analytical papers consider a unifying approach where the impact of real wireless network phenomenona is measured directly in terms of distributed control performance. 
%\if\pubMode\TechRep
%        \if\thmSlotCorrelationsFD\ref{prp:slotCorrelationsFD}
%        \if\corNakagamiFD\ref{cor:nakagamiFD}
%        \if\prfSlotCorrelationsHD\ref{prf:slotCorrelationsHD}
%        \if\ref{sec:full_duplex}\secFullDuplex
%            % TechRep
%        \else
%            \comment{ERROR 1}
%        \fi
%        \else
%        \comment{ERROR 2}
%        \fi
%        \else        
%        \comment{ERROR 3}
%        \fi
%        \else        
%        \comment{ERROR 4}
%        \fi
%\else
%    % IEEE
%\fi

In this work, we follow such unifying approach. At first, we quantify outage correlations due to random media access control for finite WSN's and for snapshots of multi agent systems. Thereafter, we consider distributed average consensus, a basic building block of distributed control,
and lay open that a thorough analysis of control performance requires knowledge of how packet losses are correlated.
%since an uncorrelated Bernoulli model with the same packet success rates may paint a different picture. 

When speaking of correlation, we mean outage correlation \cite{Talarico2018} in decorrelated fading channels (communication channels are typically located such that they are neither spatially nor temporally correlated).
%unless stated otherwise. 
The correlation we study here comes from random media access.
%which induces random sets of active nodes which are responsible for the correlation.

%Without this randomness there is no correlation for most of the links, a fact we exploit to derive our main result. Moreover, correlation decreases as spatial distance between affected nodes increases \cite{Haenggi14}. 

We consider snapshots of node deployments 
%with fixed order 
and identify two components of correlation. First, correlation between all recipients of the same transmitter, and second, correlation between all other links. Typically, the former is positive, the latter is mostly negative.
%Therefore we refer to them as \df{positive} and \df{negative} component.

The applications we have in mind all require broadcast transmission such that Request To Send/Clear To Send mechanisms cannot be applied. Examples consist of formation control \cite{Dutta2016}, flocking (cf. the references in \cite{Olfati-Saber2007}) %\addRef{ControlPaper})
or purely computational tasks like determining the network size \cite{Sluciak2013}. Literature in the former field
have been considering 
%having network models tends to impose 
oversimplified wireless network assumptions so far \cite{Dutta2016}, \cite{Sardellitti2012}.

We build our analysis on a framed slotted ALOHA media access protocol and measure the effects 
%on distributed schemes in terms of 
on the performance of an average consensus protocol. 
The simplicity of slotted ALOHA allows for exact theoretical analysis of the control performance for the given deployment. 
%Moreover, even when carrier sensing would be applied, with increasing node density carrier sensing becomes less and less beneficial.
%Moreover, even when carrier sensing is applied, with increasing node density carrier sensing becomes less and less beneficial.
Moreover, even if carrier sensing was applied, it would still become less and less beneficial with increasing node density.
For example, it was theoretically studied in \cite{Baccelli13} that the IEEE 802.11p protocol behaves like slotted ALOHA in the dense regime.





%Existing work considers mostly point process theory \cite{Haenggi14}, \cite{Kim2019}, \cite{Talarico2018} or uncorrelated links \cite{ICCCN19}.

The remainder of this work is structured as follows. In the next section we relate our study to existing work on beneficial and disadvantageous effects of correlation on communication and control performance. In section~\ref{sec:definitions} we introduce mathematical notation and the physical layer model under consideration. This is followed by section~\ref{sec:corr} where we derive an expression to compute outage correlation of random media access given an underlying fading model. This result is then used in section~\ref{sec:application} where we describe the effects correlation implies for consensus. We provide an exact and narrow performance region utilizing the so called $L^2$-joint spectral radius ($r_2$), e.g. \cite{Ogura2013}, and $L^2$-joint numerical radius ($w_2$) \cite{ICCCN19} for mean square analysis on the convergence speed of average consensus. Both measures together quite precisely render the outage correlation in terms of (discrete) control gain, fading parameter and frame length.\ %number of slots utilized. 
Compared to an uncorrelated model with the same packet loss rates, we essentially observe a beneficial impact of correlation 
on average consensus performance. We conclude our findings in section~\ref{sec:conclusion}. 
%for the most part. 
%With increasing node density carrier sensing becomes less and less beneficial, e.g. the IEEE 802.11p protocol can behave like slotted ALOHA\cite{Baccelli13}. 





==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/20_related_work.tex <==
\section{Related work}
The performance impact of correlated communication channels is studied in an extensive field of applications. It is known that correlation in general can have positive effects, e.g. on multiple-input and multiple-output capacity \cite{Benef04} or for acknowledgements \cite{Alam2012}, or drawbacks, for instance for retransmissions \cite{Ganti2009a}.
%
More specifically, other correlation types can be found which we do not consider or are ruled out in this work, e.g.
correlation between different antennas or temporal correlation \cite{Haenggi14}.

In this work, our focus is on outage correlation, that is the correlation between packet losses along different links. In the chosen slotted ALOHA media access scheme, also other types of correlation arise which implicitly affect the outage correlation and which may be subsumed under the term interference correlation.
%Namely 
This includes slot correlation (i.e. correlation between different slots within the same frame), spatial correlation and correlation between different receivers, cf.\cite{Haenggi14}.

%Existing work considers mostly point process theory \cite{Haenggi14}, \cite{Kim2019}, \cite{Talarico2018} or uncorrelated links \cite{ICCCN19}.

Interference correlation can be studied for fixed node configurations or for networks 
modeled as point processes as studied in \cite{Ganti2009a}, \cite{Haenggi14}, \cite{Krishnan2017}. 
Recently, outage correlation has been investigated in a finite point process setting (Binomial, Poisson and Thomas processes) under Rayleigh Fading \cite{Talarico2018}. 
Although the authors allow for slotted ALOHA, they are mainly concerned with the effects of the spatial differences generated by the three point processes; concrete node deployments are not considered. 
The work \cite{Kim2019} is set also in a point process setting where spatial interference correlation is investigated. Instead of computing the correlations exactly, the authors elaborate approximations. 

Our analytical derivations significantly differ from the aforementioned works. Here we are specifically interested in the impact of outage correlation for a finite, fixed node deployment with respect to convergence speed of average consensus using broadcast communication.

For convergence speed of average consensus under channel correlation and wireless network constraints other work exist. In\cite{Chan10}, consensus has been considered under fast fading where correlated outages (mainly due to fading) are mentioned without being quantified. In \cite{Kar2009}, \cite{Silva11} abstract correlations can be handled in the consensus framework, however, neither a physical model nor a media access model is provided. Also the mean square disagreement measures used there are upper bounds only. In our work we use a different upper bound, $w_2$, which very well matches the shape of the exact measure $r_2$ characterizing (exponential) mean square stability, cf. \cite{ICCCN19}. 

Finally, the outage probabilities for Nakagami-m fading we plug into our model (Corollary~\ref{cor:nakagamiHD})
stem from \cite{Nakagami12}, one of the few papers analyzing fixed node deployments. However, as opposed to our work, correlation is not considered in that reference.
%An early work meantioning the exactness of $r_2$ but rather analyzing an upper bound for the sake of simplicity is \cite{Boyd2006}. 

%\cite{Dutta2016}
%\cite{Sardellitti2012}

==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/30_theory.tex <==
%\section{Physical layer network model}
\section{Definitions and model assumptions}\label{sec:definitions}
\subsection{Matrix, vector and other notation}
\label{notation_section}
%$\N = \left\{ 1, 2, \dots \right\}$ set of natural numbers, $\R, \C$ field of real respectively complex numbers.
For vectors $x\in \R^n$ we adopt the Euclicean norm $\norm{x} = \sqrt{\sum_{i=1}^{n} x_i^2}.$ By $\one \in \R^n$ we denote the vector of all ones. The identity matrix on $\R^n$ is denoted by $I_n,$ whereas by $\Pi$ we denote the projection matrix $I_n - \frac{\one \one^T}{n}.$
%
%The cartesian basis vectors are denoted by $e_i\in \R^n, i = 1, \dots, n$, i.e. $e_i = (0, \dots, 0, 1, 0, \dots 0),$ where the one is located at the $i$-th position.


The Kronecker delta is denoted by $\delta_{ij}$, i.e. $\delta_{ij} = 1$ if $i = j$ and $\delta_{ij} = 0$ otherwise; $\delta_{i\ne j}$ is short for $1-\delta_{ij}.$  For two matrices $A,B \in \R^{n\times n}$ we denote by $A\otimes B$ the Kronecker product of $A$ and $B,$ i.e. for indices of the form $I = n\cdot (i-1)+k,\; J=n\cdot (j-1) +l,\; 1 \le i,j,k,l \le n,$ we have $(A\otimes B)_{IJ} = a_{ij}b_{kl}.$ 

By $\ind(x\ge0)$ we denote the unit step function on $\R$, i.e. $\ind(x\ge0)$ is equal to one if $x\ge0,$ %and is equal to 0 otherwise. 
and vanishes otherwise.


Let $X$ be an arbitrary set and $n\in \N.$ By $X^n$ we denote the $n$-fold cartesian product $X \times \dots \times X.$ 
We will use ordered tuples over sets $X$ 
%We next introduce ordered tuples
as follows: For a sequence $(a_\nu)_{\nu \in \N} \subset X$ and a finite index set $J \subset \N$ we denote by $[a_\nu]_{\nu \in J}$ the tuple $(a_{\nu_{1}}, \dots, a_{\nu_{\abs{J}}}) \in X^{\abs{J}}$ where 
$\nu_1 = \min J, \mbox{ and }  \nu_{k+1} = \min J\setminus\{\nu_1, \dots, \nu_k\}, \ds k = 1, \dots \abs{J} -1.$

\subsection{Physical layer model}
We assume $n \ge 3$ nodes $u_1, \dots, u_n$ located at fixed positions $(x_1, \dots, x_n) \in \R^{3n}$ relative to a possibly moving frame of reference. A transmission between two nodes $u_i$ and $u_j$ is subject to path loss with a path loss coefficient of $\alpha_{\text{PL}} \ge 2$. For a transmission distance $d$ the average received power is thus proportional to $1/d^{\alpha_{\text{PL}}}$
in the far field. 

Let $\mu_{ij}^{-1}, \, 1 \le i, j \le n,\; i \ne j,$ be the average power of a transmission from $u_i$ received at $u_j$.
%if $u_i$ is solely transmitting (the notation shall not be affected if there are actually other nodes sending in which case $\mu_{ij}^{-1}$ is just the received power fraction due to node $u_i$).
If $u_i$ transmits with power $q_i,$ we have 
$\mu_{ij} = \frac{1}{q_{i}}(\norm{x_i - x_j}/r_0)^{\alpha_{\text{PL}}}$, where $r_0$ is a reference distance. Denoting the wavelength of the carrier wave by $\lambda$ we choose $r_0 = \lambda/4\pi$ such that we arrive at Friis free space equation in case of a path loss coefficient of $2.$

Here we study communication under the effect of narrow band fast fading. This means that the instantaneous received power $P_{ij}$ of a transmission between $u_i$ and $u_j$ is a non-negative random variable with expectation $\mu_{ij}^{-1}$. 
Further, we assume independent block fading (IBF), i.e. $P_{ij}$ is constant during a packet transmission and power variables belonging to different channels are mutually independent.
Later we employ the Nakagami fading model, i.e., the random variable $P_{ij}$ is Gamma distributed with probability densitiy function (pdf) 
\begin{equation}
%f_{ij}(x) = \frac {2m^{m}}{\Gamma (m)\Omega ^{m}} x^{2m-1}\exp \left(-{\frac {m}{\Omega }}x^{2}\right)
	\label{eqn:naka_pdf}
	%f_{ij}(x) = \text{ind}(x>0) \frac {m_{i}^{m_{i}}\mu_{ij}^{m_{i}}}{q_{ij}^{m_i}\Gamma (m_i)} x^{m_{i}-1}\exp \left(-m_{i}x\mu_{ij}/q_{ij} \right)
	f_{ij}(x) = \ind(x\ge0) \frac {m_{i}^{m_{i}}\mu_{ij}^{m_{i}}}{\Gamma (m_i)} x^{m_{i}-1}\exp \left(-m_{i}x\mu_{ij} \right)
\end{equation}
where $m_i  \in \N$ are integer\footnote{In general, Nakagami fading only requires $m_i \ge 1/2,$ however since we build on \cite{Nakagami12}, we can only handle integer values.} shape parameters. 
%$\mu_{ij}:= \frac{1}{p_{ij}}(4 \pi \norm{x_i - x_j}/\lambda)^2,$
%$\mu_{ij}:= \frac{1}{p_{ij}}(\norm{x_i - x_j}/r_0)^{\alpha_{\text{PL}}},$
However, our calculations of the structure of correlation due to random media access are valid in a very general setting regardless of path loss and fading (cf. state coefficients of Theorem~\ref{prp:slotCorrelationsHD} and 
\if\pubMode\IEEE
     \cite[Theorem~\thmSlotCorrelationsFD{}]{TechRep}
\else
    \ref{prp:slotCorrelationsFD}
\fi).
We incorporate Nakagami fading as special case in Corollary~\ref{cor:nakagamiHD} and 
\if\pubMode\IEEE
     \cite[Corollary~\corNakagamiFD]{TechRep}
\else
    \ref{cor:nakagamiFD}.
\fi.


The success rate of a message transmission is modeled with outage probability under the signal to interference plus noise ratio (SINR) model. For a transmission from $u_i$ to $u_j$ all other currently ongoing transmissions will be considered as noise. Thus, we relate the received power over noise plus all other interfering transmissions as
\begin{equation}
	\label{eqn:SINR}
	\mathrm{SINR}_{ij} = \frac{P_{ij}}{N + \sum_{\nu \in V \setminus \{ i,j \}} P_{\nu j}}
\end{equation}
where $N$ is a constant thermal noise term and $V$ the set of node indices of all currently transmitting nodes. Let the receiving node $u_j$ be silent. Then we say the transmission has an outage if $\mathrm{SINR}_{ij}$ falls below a system specific \df{threshold} value $\theta > 0$ and the probability of a successful packet transmission from $u_i$ to $u_j$ is $\Pr[\mathrm{SINR_{ij}} \geq \theta].$
The case when $u_j$ is also transmitting will be discussed in the context of the slot model in the next section.

%For media access in one round of the consensus protocol time is divided into $m$ slots. Each node chooses one of the $m$ slots uniformly distributed (i.e.\ with probability $1/m$) and independent of the other nodes' choices.

%\comment{Copied from ICCCN paper for exemplary purposes, has to be adapted!!! Continue 
%reading in the next subsection} 
%\color{blue}
%\label{subsection:SINR}
%We consider received power in a potential collision domain of $n$ nodes $u_1, \dots, u_n$ with a path loss coefficient $2.$ We consider that received power in the far field is proportional to transmit power scaled by a factor $\frac{1}{d^2}.$ One example is Friis equation with antenna gain factor $1$, i.e. received power $P_{{RX}}$ (in the far field) given by $P_{{RX}} = P_{{TX}}\cdot (\lambda/(4 \pi d))^2$ where $P_{{{TX}}}$ is the common transmit power, $d$ the sender receiver separation and $\lambda$ the carrier wave length.
%
%Let $P_{{RX}}^{ij}$ be the power received by $u_j$ of a transmission from $u_i$. We express interference from all other ongoing transmissions by the SINR model:
	%$$\text{SINR} = \frac{P_{RX}^{ik}}{N + \sum_{u_j \in V \setminus \{ u_i \}} P_{RX}^{jk}},$$
%	$$\text{SINR} = \frac{P_{RX}^{ik}}{N + \sum_{u_j \in V \setminus \{ u_i \}} P_{RX}^{jk}},$$
%where $N$ is a constant thermal noise term and $V$ is the set of all nodes transmitting at the moment. Thermal noise is given by $N = B T k_B$ where $B$ is the utilized bandwidth in Hz, $T$ the temperature in Kelvin and $k_B$ the Boltzmann constant.
%
%Packet error is modeled according to outage probability, i.e. for correct packet reception SINR has to be greater or equal a system constant $\theta$. We set $\theta$ according to Shannon capacity formula $C=B \log_2 (1+\text{SNR})$. We approximate interference as noise. Thus, given bandwidth $B$, utilized bit rate $C$ and considering $I+N$ as noise yields $\theta = 2^{C/B} - 1$. \begin{newcont} A fading margin can also be added. This, however, does not change anything for our mathematical derivation and is left out to keep the derivation uncluttered. \end{newcont}
%
%Let $m$ be a number of so called \df{slots} available in each round of the consensus protocol, and first let $m \in \N$. Slotted ALOHA means here, that at each step of the consensus iteration, all nodes independently choose one of $m$ disjoint collision domains with probability $\frac{1}{m}.$ 

%Under Rayleigh fading, the probability density function (pdf) $f(x)$ of the received power $P_{RX}^{ij}$ is given by $f(x) = \mu_{ij} e^{-\mu_{ij} x} \cdot \ind$, \mbox{ where } $\ind = \left\{\begin{aligned} &1, &\mbox{ if } x > 0 \\ &0, &\mbox{ else, }   \end{aligned}$

\color{black}

\section{Outage correlation due to media access}
\label{sec:corr}
To determine the coefficient of correlation of transmission success between different node pairs, it suffices to specify expectation and covariance, which is the concern of this section.
%\subsection{Introductory Example}
%Consider three nodes $u, v_1, v_2,$ such that $\n{uv_1} = \n{uv_2}.$

%\subsection{MAC layer: slotted ALOHA model in the full duplex case}
%In addition to the physical layer model, we now assume the following slot model for broadcast transmission. 

%For our analysis we choose a prototypical media access scheme, a variant of slotted ALOHA we call \df{slot picking (ALOHA)}. 
%It is the same slotted ALOHA model (\comment{IFS ignored}) as used in \cite{Baccelli13} to describe the behavior of the more sophisticated carrier sense multiple access (CSMA) scheme of IEEE 802.11p in the \df{dense network scenario}. The connection of the latter with slot picking is summarized in Appendix \addRef{}, here we will discuss the former. The correlation effects we observe are not limited to slot picking ALOHA alone. Instead our method can be carried over to  other variants like spatial and opportunistic ALOHA described in \addRef{}; the correlation is still nonzero.
%and CSMA properties (backoff etc.) are not visible any more.
 
In addition to the physical layer model, we now assume that the nodes perform the following variant of slotted ALOHA for broadcast transmission which guarantees that each node transmits exactly once during a beacon period. Let $\tau$ be the duration of the beacon time interval in milliseconds (ms) which is called a \textit{frame.} 
%Every $\tau$ ms each node has a packet to transmit. 
Each frame is divided into a number $m$ of time intervals called \textit{slots}, where $m \in \N$ is chosen such that each packet can be transmitted in $\tau/m$ ms. At the beginning of each frame, each node randomly chooses exactly one slot with equal probability. Transmission from node $u_i$ to node $u_j$ is successful if it is successful in the chosen slot. Otherwise the packet from $u_i$ to $u_j$ is considered lost in this beacon interval.

%Let $\tau$ be the duration of the beacon time interval in milliseconds (ms) which is called a \textit{frame.} Every $\tau$ ms each node has a packet to transmit. Each frame is devided into a number $m$ of time intervals called \textit{slots}, where we require $m \in \N$ to be chosen such that each packet can be transmitted in $\tau/m$ ms. At the beginning of each frame each node randomly choses exactly one slot with equal probability. Transmission from node $u_i$ to node $u_j$ is successfull if it is successful in the chosen slot. Otherwise the packet is considered lost.

%Denote by $\theta \in \R_+$ the SINR threshold.
Our derivation requires\footnote{Cf. Remark \ref{rem:thm} and Section \ref{sec:parameters}. The assumption $\theta \ge 1$ is commonly used in singular antenna systems, \cite{Clazzer2017}. } $\theta \ge 1$ and $N>0$ Watt. Let us further introduce $n$ independent random variables $S_1,\dots, S_n$ representing each node's choice of slot - all equally likely - i.e. $S_i \sim unif(\{1, \dots, m\}), \; i = 1 ,\dots n,$ (uniform distribution).
%Denote by $P_{ij}, \, 1 \le i, j \le n,\; i \ne j,$ the power received at node $u_j$ if some different node $u_i$ is solely transmitting, subject to path loss and fading (the notation shall not be affected if there are actually other nodes sending in which case $p{ij}$ is just the received power fraction due to node $u_i$). In this work we will consider Gamma distributed (Nakagami fading) and (non-central) chi-square distributed (Ricean fading) powers. However, theoretical considerations are limited to Nakagami fading to keep mathematics tractable, although the slot model yields general expressions independent of the fading distribution (see Prop. \ref{prp:slotCorrelationsFD}). 

Moreover we assume the power variables $P_{ij}$ - e.g. $P_{ij} \sim f_{ij},$ cf. (\ref{eqn:naka_pdf}) - to be independent (IBF assumption) and also to be independent from the slot variables. We can now express power and interference in slot $k, \; 1 \le k \le m:$
	$$P_{ij}^{k} := \delta_{S_i k} P_{ij} \ds \mbox{ and }\ds I_{ij}^k := \sum_{\substack{l=1 \\ l\ne i,j}}^{n}P_{lj}^{k}.$$
Let us introduce random variables for excess of the SINR threshold in slot $k$ and in any slot respectively:
	$$X_{ij}^k := \ind\left(\frac{P_{ij}^k}{N + I_{ij}^k}\ge \theta  \right) \ds \mbox{ and } \ds X_{ij} := \sum_{k=1}^{m} X_{ij}^k.$$
	Clearly, from the definition of $P_{ij}^k$ and the fact that $\theta, (N + I_{ij}^k) >0$ we have $X_{ij}^k = \delta_{S_i k} \cdot X_{ij}^k,$ thus $X_{ij} = X_{ij}^{S_i}.$

	There are two further practial aspects we have to consider: Sending nodes cannot receive (singular antenna case) and multiple receptions at some node at the same time (i.e. in the same slot) are impossible in our model since $\theta \ge 1.$  %will only model the former aspect in our formal treatment 
	%which we call the 
	We call the former aspect the 
	\df{half-duplex} case. 
%However, we keep track of the latter case in simulations and show (\comment{verify!!}) that this happens rarely such that our analysis is still meaningful. \comment{Maybe also add estimates somewhere}. 
%
We define successful \df{full-duplex} packet transmission from node $u_i$ to $u_j$ to be the event $X_{ij} = 1.$ In words: We ignore whether the receiver is sending or not when checking for excess of the SINR ratio.
	
	In this sense, we model successful half-duplex packet reception $Y_{ij}, \, 1 \le i, j \le n,\; i \ne j,$ as Bernoulli variable having the property to vanish if $u_i$ and $u_j$ chose the same slot and to coincide with $X_{ij}$ otherwise:
\begin{equation} \label{eqn:X_Y}Y_{ij} := (1-\delta_{S_i S_j}) \cdot X_{ij} \ds\ds 1 \le i,j \le n, i\ne j.\end{equation}
%It follows immediately that 
	%$$\E Y_{ij}Y_{kl} = \E \left[ X_{ij}X_{kl} \mid S_i \ne S_j, \; S_k \ne S_l \right].$$
Our goal is to determine how successful transmissions are correlated. Therefore, we calculate the covariances $\cov(Y_{ij}, Y_{kl})$ and begin with the mixed moments of the $X_{ij}$'s (full-duplex case) which are of special importance.
By the law of total probability we can decompose the mixed moments $\E X_{ij}X_{kl},\, i \ne k,$ into a weighted sum of the conditioned mixed moments
	\begin{equation}\label{eqn:decomposition1_mixed_moments}\frac{1}{m} \cdot \E[X_{ij}X_{kl}\vert S_{i} = S_{k}] + (1-\frac{1}{m})\E[X_{ij}X_{kl}\vert S_{i} \ne S_{k}]\end{equation}
motivating the form of the main result of this section which needs a little technical preparation. The conditioned mixed moments of the $X_{ij}$'s, as well as those of the $Y_{ij}$'s, lead - up to normalization - to expressions of the form (\ref{eqn:formulaSameSlot}) and (\ref{eqn:formulaDiffSlot}) which we will now describe:
%An analogous decomposition obviously holds for $Y_{ij},$ together motivating the proposition below which needs a little technical preparation. The conditioned mixed moments of both $X_{ij}$ and $Y_{ij}$ lead to expressions of the following form:
Denote by $b_\nu \in \left\{ 1,\dots, m \right\}$ realizations of the slot random variables $S_\nu$ which we call \df{micro states}. Consider for instance a transmission from node $u_i$ to $u_j.$ %The interference pattern of all other disturbing nodes can be summerized by 
The pattern of the micro states contributing to the interference for this transmission can be summerized by
simpler \df{macro state} variables $c_\nu \in \{0,1,2\}, \nu \ne i,j.$ % representing a collection of micro states.
Consider, e.g., a further node $u_k$ under the condition $S_i \ne S_k,$ i.e. $u_i$ and $u_k$ have chosen different slots. In one possible interpretation $c_\nu = 0$ may stand for all realizations of the event $S_\nu \ne S_i, S_k,$ the case $ c_\nu = 1$ might stand for all realizations of $S_\nu  = S_i$ and $c_\nu = 2$ for all realizations of $S_\nu = S_k.$
%Each $c_\nu$ denotes a slot macro state representing the interference pattern while the functions $\phi(c)$ and $\psi(c)$ denote the weights assigned to the total state $c$. We call these functions \df{state weights}
%E.g. $c_\nu = 0$ may stand for all realizations of the event $S_\nu \ne S_i.$ %Each $c_\nu$ denotes a slot macro state representing the interference pattern while the functions $\phi(c)$ and $\psi(c)$ denote the weights assigned to the total state $c$. We call these functions \df{state weights}
In general, for a subset $J$ of $\mathcal N:= \left\{ 1, \dots, m \right\}$ we denote by $c$ the tuple $[c_\nu]_{\nu \in J},$ the \df{total (macro) state}. We express the number of micro states represented by this total state by functions $\phi(c)$ and $\psi(c)$ which we call \df{state weights}.

%Now assume that in the same frame there is a second transmission going on from some node $u_j$ to $u_k$. 
Now let us take a look at some potential receiver $u_l$ of $u_k$'s transmission. The idea in the calculation of ((un-)conditioned) mixed moments of $X_{ij}$ and $X_{kl}$ is to condition on the slot variables until all $S_{\nu}$ have been replaced by micro states $b_\nu.$ The mixed moments then expand into a sum of weighted probabilities. When exploiting common interference terms, the probability summands split up into a product of two separate probabilities in virtue of the  independence
%\footnote{there is one exceptional case which is the reason for the requirement $\theta \ge 1.$}
(IBF assumption). For either of the two factors we use the terminology \df{state coefficient} - symbolized by either $\alpha_{ijkl}(c)$ or $\beta_{ijkl}^{(d)}(c).$ These probabilities depend, of course, on the fading model (cf. Corollary~\ref{cor:nakagamiHD}). State weight and state coefficients are also called \df{state functions}. %A collection of state functions by using the function symbol without sub script, super script and function argument as on the lefthand side in (\ref{eqn:formulaSameSlot}), (\ref{eqn:formulaDiffSlot}). 

For $i \ne j, k \ne l, (i,j) \ne (k,l),$ and for a finite index set $J \subset \mathcal N$ %we can now define
we now introduce expressions allowing for a quite general treatment of outage correlation expressions\footnote{The summation appearing in (\ref{eqn:formulaSameSlot}) and (\ref{eqn:formulaDiffSlot}) is meant to expand into a $\abs{J}$-fold sum over $c_\nu,\, \nu \in J,$ e.g. $\sum_{\substack{c_\nu=0 \\\nu \in \mathcal N}}^{1}(\dots) = \sum_{\nu_1, \dots, \nu_n = 0}^1(\dots)$.}
%\footnote{the product with subsequent summation appearing in (\ref{eqn:formulaSameSlot}) and (\ref{eqn:formulaDiffSlot}) is meant to expand into a $\abs{J}$-fold sum over $c_\nu,\, \nu \in J.$}
\begin{equation}\begin{aligned}\label{eqn:formulaSameSlot}
		%\Phi_{ijkl}  :=  \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijk}(c)\cdot \alpha_{kli}(c) \end{aligned}
		%\Phi_{ijkl}  :=  \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijkl}(c)\cdot \alpha_{klij}(c)
		%\Phi_{ijkl}^{\mathcal N\setminus \left\{ i,k \right\}}  :=  \prod_{\substack{\nu \in J}}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijkl}(c)\cdot \alpha_{klij}(c)
		%\Phi_{ijkl}^{J}(\phi, \alpha):=  \prod_{\substack{\nu \in J}} \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijkl}(c)\cdot \alpha_{klij}(c)
		\Phi_{ijkl}^{J}(\phi, \alpha):=  \sum_{\substack{c_\nu=0\\ \nu\in J}}^{1}\phi(c)\cdot \alpha_{ijkl}(c)\cdot \alpha_{klij}(c)
 \end{aligned}\end{equation}
and
\begin{equation}
	\label{eqn:formulaDiffSlot}
	%\Psi_{ijkl}(\psi, \beta) :=\prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c),
	\Psi_{ijkl}^J(\psi, \beta) :=\sum_{\substack{c_\nu=0\\ \nu \in J}}^{2}  \psi(c)\cdot \beta_{ijkl}^{(1)}(c) \cdot \beta_{klij}^{(2)}(c),
\end{equation}
	%$$\Psi_{ijkl} :=\prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c),$$ 
where $\phi(c), \psi(c), \alpha_{xyzw}(c)$ and $\beta_{xyzw}^{(d)}(c)$ are functions of 
	%$c = (c_\nu) \in   \left\{ 0,1,2 \right\}^{n-2+\delta_{ik}},$ 
	%$$c = (c_1, \dots, c_{\mu-1},c_{\mu+1},\dots, c_{M-1}, c_{M+1},\dots, c_n),$$
	%and where $\mu = \mbox{min}(i,k), M = \mbox{max}(i,k).$ 
$c = [c_\nu]_{\nu \in J} \in   \left\{ 0,1,2 \right\}^{\abs J}$ (see section \ref{notation_section}).
E.g. for $J = \mathcal N \setminus \left\{ i,k \right\}$ we have $[c_\nu]_{\nu \in J} = (c_1, \dots, c_{\mu-1},c_{\mu+1},\dots, c_{\hat \mu-1}, c_{\hat \mu+1},\dots, c_n),$ where $\mu = \mbox{min}(i,k)$ and $\hat \mu = \mbox{max}(i,k).$ 
In case of the calculation of $\Phi_{ijkl}^J$ we always have $c_\nu \ne 2$ such that there $[c_\nu]_{\nu \in J} \in   \left\{ 0,1 \right\}^{\abs J}$ holds true.


We are now ready to formulate our covariance result for the $Y_{ij}$'s. An analogous result for the $X_{ij}$'s can be found in 
\if\pubMode\IEEE
the Appendix of \cite{TechRep}.
\else
Appendix~\ref{sec:full_duplex}.
\fi
%In this section we determine the covariance for the - from practical point of view - more significant half duplex case. 
From (\ref{eqn:X_Y}) we obtain for $i\ne k$ and $k\ne l$
	%$$ \begin{aligned}\E Y_{ij} Y_{kl} = \; &\Pr(S_i \ne S_j \mbox{ and } S_k \ne S_l) \\ &\cdot \E [X_{ij} X_{kl} \mid S_i \ne S_j, S_k \ne S_l]. \end{aligned}$$

	$$ \begin{aligned}\E [Y_{ij} Y_{kl}] = \left(1-\frac{1}{m}\right)^{2-\delta_{kj}\delta_{li}} \E [X_{ij} X_{kl} \mid S_i \ne S_j; S_k \ne S_l]. \end{aligned}$$
	%Note that the prefactor is independent of the actual number of (different) elements in $\left\{ i,j,k,l \right\}.$
In the following Theorem we treat the cases $S_i = S_k$ and $S_i \ne S_k$ separately,  cf. (\ref{eqn:decomposition1_mixed_moments}).
\begin{thm}[Half-duplex covariances]
\label{prp:slotCorrelationsHD}
\item Let $n \ge 3, \theta \ge 1,N > 0, i \ne j, k \ne l,$ and let $(i,j) \ne (k,l).$ (a)\; We have for $j\ne k$ and $i\ne l$
%\begin{abc}
%\item
%$i\ne k:$

$$  \begin{aligned} \E &\left[ X_{ij}X_{kl} \mid S_i = S_k; S_i \ne S_j; S_k \ne S_l \right] \\&= \frac{ (1-\delta_{l j})\cdot \Phi_{ijkl}^{\mathcal N \setminus\left\{ i,j,k,l \right\}}(\phi, \alpha)}{m^{n-4+\delta_{ik}}},  \end{aligned} $$ 

where the state weight of $c = [c_\nu]_{\nu\in \mathcal N\setminus \left\{ i,j,k,l \right\}}$ is given by
	\begin{equation}\label{eqn:state_weight_a_HD}\phi(c) = \prod_{\nu \in \mathcal N \setminus \left\{ i,j,k,l \right\}}(m-1)^{1-c_\nu},\end{equation}
	the state coefficients $\alpha_{xyzw}(c)$ are given by 
 	\begin{equation*}
		\begin{aligned}
		\Pr\left(\frac{P_{xy}}{N+\sum\limits_{\nu\ne x,y,z,w}^{}c_\nu P_{\nu y} + (1-\delta_{xz})P_{zy}} \ge \theta\right).		\end{aligned}
	\end{equation*} 
In particular, $\E[ Y_{ij}Y_{il}]$ can be expressed this way, hence for $j \ne l$
	\begin{equation}\label{eqn:cov_a_HD}cov(Y_{ij},Y_{il}) = \left(1-\frac{1}{m}\right)^2\cdot \frac{\Phi_{ijil}^{\mathcal N \setminus\left\{ i,j,l \right\}}}{m^{n-3}}(\phi, \alpha) - \E [Y_{ij}]\E[ Y_{il}].\end{equation}
%\item
(b) Let $J' = \{i,j,k,l\}$, let $J'' = \{i,k\}$ if $\abs{J'} =4$ and $J''=J'$ else. Moreover, let $J'''=\{i,j,k\}$ if $\abs{J'}=4$ and $J''' = J'$ otherwise. Then, for $k\ne i,$ % and $J^{\mathcal{C}} = \left\{ i,j,k,l \right\},$
we have, 
	$$ \begin{aligned}&\E [X_{ij}X_{kl}\vert S_i \ne S_j, S_k;\, S_k \ne S_l]  = \frac{\Psi_{ijkl}^{\mathcal N \setminus J''}(\psi, \beta)}{M}
			%&= \frac{1}{(m-1)m^{n-1}} \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
			,\end{aligned}$$
		%where $M = m^{n-2}$ if $\abs{J'} = 2,$  $M=m^{n-3}$ if $\abs{J'}=3$ and $M=m^{n-3}\cdot(m-1)$ if $\abs{J'}=4$. Hence,
		where $M = m^{n-\abs{J'}}$ if $\abs{J'} = 2, 3$  and $M=m^{n-3}\cdot(m-1)$ if $\abs{J'}=4$. Moreover, for $k \ne i,$
        \begin{equation}\label{eqn:cov_b_HD}\begin{aligned} &\cov(Y_{ij}, Y_{kl}) = 
		%(1-\frac{1}{m})^{2-\delta_{kj}\delta_{li}}\left[ \frac{\delta_{l\ne i}\delta_{l\ne j}\delta_{j\ne k}\Phi_{ijkl}^{\mathcal N \setminus J'}(\phi, \alpha)}{m^{n-4+\delta_{ik}}}\right.\\
		(1-\frac{1}{m})^{2-\delta_{kj}\delta_{li}}\left[ \frac{\delta_{\abs{J'},4} (m-1)\Phi_{ijkl}^{\mathcal N \setminus J'}(\phi, \alpha)}{m^{n-3}}\right.\\
			%&  + \frac{(m-1)^2}
			&   +\left. %(1-\frac{1}{m})^{2-\delta_{kj}\delta_{li}}
            \left[\frac{m-1}{m} \delta_{\abs{J'},4} + \frac{m-2}{m-1}\delta_{l,j} +
            \delta_{l\ne j}\delta_{\abs{J'}\ne 4}\right]
			\frac{\Psi_{ijkl}^{\mathcal N \setminus J''}(\psi, \beta)}{M}\right] \\
			& - \E [Y_{ij}]\cdot \E [Y_{kl}], 
			%\frac{1}{M}\cdot \Psi_{ijkl}^{\mathcal N \setminus J''}(\psi, \beta)\right] - \E Y_{ij} \E Y_{kl}, 
			\end{aligned}\end{equation}
	    where $\Phi_{ijkl}(\phi, \alpha)$ depends on the state functions of part (a) whence $\Psi_{ijkl}(\psi, \beta)$ depends on the state weight
	    \begin{equation}\label{eqn:state_weight_b_HD}\psi(c) =  \left[\delta_{c_l\ne 2}\cdot  \delta_{c_j\ne 1} \cdot( m-1)^{\delta_{0,c_j}}\right]^{\delta_{\abs{J'},4}} \prod_{\substack{\nu = 1\\ \nu \not\in J'''}}^n (m-2)^{\delta_{c_\nu, 0}}\end{equation}
	and on the state coefficients
			%\alpha_{i'j'}(c) &: = \Pr\left(\frac{P_{i'j'}}{N+\sum_{\nu\ne i',j'}^{}c_\nu P_{\nu j'}} \ge \theta\right),\\
			%\alpha_{xy}(c) &: = \Pr\left(\frac{P_{xy}}{N+\sum_{\nu\ne x,y}^{}c_\nu P_{\nu y}} \ge \theta\right),
		$$\beta_{xyzw}^{(d)}(c)  = \Pr\left(\frac{P_{xy}}{N+\sum_{\nu\ne x,y,z}^{}\delta_{c_\nu d} P_{\nu y}} \ge \theta  \right),$$
where $c = [c_\nu]_{\nu\in \mathcal N\setminus J''}$,  $d = 1,2.$ 
 
%\end{abc}
\end{thm} 
\begin{proof}
\if\pubMode\IEEE
    The proof utilizes the conditioning and macro state techniques sketched above. For details see \cite[Appendix]{TechRep}.
    %Due to space limitations the proof is part of the technical report \cite[Appendix]{TechRep}.
\else
    See Appendix \ref{prf:slotCorrelationsHD}.
\fi
\end{proof}
\begin{rem}
	\label{rem:thm}
	\begin{rom}
	\item The requirement $\theta \ge 1$ is used in the case $l = j$ and yields the $(1-\delta_{lj})$ factor.
	%\item In case $m=1$ we have $\Phi_{ijkl} = \E X_{ij} \E X_{kl}$ \comment{(verify!)} and so ``everything is uncorrelated as expected'' \comment{(verify!!)}
	\item In case $m=1$ there is no outage correlation in the full-duplex case, i.e. $\cov(X_{ij}, X_{kl}) = 0$ for $(i,j) \ne (k,l).$ 
	\item Typically, the covariance component given by (a) seems to be stronger than the one given by (b). 
	For the correlations this observation does not hold; we may merely assert that the component due to (a) is typically positively correlated while the one due to (b) is correlated mainly negatively, 
	cf. Figure~\ref{fig:correlation}.
	%\item Correlation increases as $m$ increases. \comment{not fully true} \comment{What about $Y$??}
	\item Since the summations can get large it is important to efficiently implement the sums. E.g. $\sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^1 \left( \dots \right)$ can be implemented using a loop from 1 to $2^{n-2}$ over a \textit{single} integer variable $i$ and accessing the ``components'' $c_{\nu}$ of $i$ by bitwise operations (bit-shift).
 
	\end{rom}
\end{rem} 

\begin{rem}
\label{rem:backward_compatibility}
Using Rayleigh fading in the slot model we recover the success probabilities of \cite{Nakagami12} (full-duplex) and \cite{ICCCN19} (half-duplex). The calculation is provided in 
\if\pubMode\IEEE
    \cite{TechRep}.
\else
    Appendix \ref{prf:backward_compatibility}.
\fi
Moreover, a similar argument is part of Corollary \ref{cor:nakagamiHD}.
\end{rem} 
To incorporate Nakagami fading (cf. (\ref{eqn:naka_pdf})) we introduce for convenience a further notation, which is the link to \cite{Nakagami12}: For a finite index set $J\subset \mathcal N$ and an $\R$-valued tuple $\xi = [\xi_\nu]_{\nu\in J}$%,\; J = \mathcal{N}\setminus \left\{ i,j \right\},$
 let

%$$\begin{aligned}\gamma_{i'j'}(x) &= e^{-\theta\cdot m_{i'} \cdot \mu_{i'j'} \frac{N}{q_{i'j'}}} \sum_{s=0}^{m_{i'}-1}\left( \theta \cdot m_{i'} \cdot \mu_{i'j'} \frac{N}{q_{ij}} \right)^s \\& \cdot \sum_{t=0}^{s}\frac{(\frac{N}{q_{ij}})^t}{\left( s-t \right)!}   \cdot \sum_{\substack{\ell_\nu \ge 0\\ \sum\limits_{\nu \ne i,j}\ell_\nu = t}}\prod_{\nu \ne i,j}\left[ \left( 1-x_{\nu} \right)\delta_{0\ell_\nu} \right. \\ &\ds\ds +\left. \frac{x_{\nu}\Gamma\left( \ell_\nu + m_\nu \right)\left( \frac{q_{\nu j}}{q_{ij} \mu_{\nu j}} \right)^{\ell_\nu}}{\ell_{\nu}! \Gamma(m_\nu)\left( \theta\frac{m_i}{m_\nu}\frac{\mu_{ij}}{\mu_{\nu j}}\frac{q_{\nu j}}{q_{ij}}+1 \right)^{m_\nu+\ell_\nu} }  \right] \end{aligned}$$

$$\begin{aligned}\gamma_{xy}^J(\xi) &= e^{-\theta\cdot m_{x} \cdot \mu_{xy} N} \sum_{s=0}^{m_{x}-1}\left( \theta \cdot m_{x} \cdot \mu_{xy} N \right)^s \\& \cdot \sum_{t=0}^{s}\frac{(\frac{q_{x}}{N})^t}{\left( s-t \right)!}   \cdot \sum_{\substack{\ell_\nu \ge 0\\ \sum\limits_{\nu \in J}\ell_\nu = t}}\prod_{\nu \in J}\left[ \vphantom{\frac{a^2}{b^2}}\left( 1-\xi_{\nu} \right)\delta_{0\ell_\nu} \right. \\
%&\ds\ds +\left. \frac{\xi_{\nu}\cdot \left( \ell_\nu + m_\nu +1 \right)!\left( \frac{1}{m_\nu q_{x} \mu_{\nu y}} \right)^{\ell_\nu}}{\ell_{\nu}! \cdot (m_\nu+1)!\left( \theta\frac{m_x}{m_\nu}\frac{\mu_{xy}}{\mu_{\nu y}}+1 \right)^{m_\nu+\ell_\nu} }  \right].
&\ds\ds +\left. \left(\begin{aligned} \ell_\nu + &m_\nu -1\\ &\ell_{\nu}\end{aligned}\right)\cdot \frac{\xi_{\nu}\cdot\left( \frac{1}{m_\nu q_{x} \mu_{\nu y}} \right)^{\ell_\nu}}{\left( \theta\frac{m_x}{m_\nu}\frac{\mu_{xy}}{\mu_{\nu y}}+1 \right)^{m_\nu+\ell_\nu} }  \right].
 %&\ds\ds +\left. \left(\begin{aligned} \ell_\nu + &m_\nu +1\\ &\ell_{\nu}\end{aligned} \right)\cdot\frac{\xi_{\nu}\cdot \left( \frac{1}{m_\nu q_{i} \mu_{\nu j}} \right)^{\ell_\nu}}{\left( \theta\frac{m_i}{m_\nu}\frac{\mu_{ij}}{\mu_{\nu j}}+1 \right)^{m_\nu+\ell_\nu} }  \right]\\
  \end{aligned}$$

 
\begin{cor}[Nakagami fading expectations and covariances]
\label{cor:nakagamiHD}
In the half-duplex model under Nakagami fading with pdf (\ref{eqn:naka_pdf}) the expectation for the link $u_i u_j,\, i \ne j,$ is given by
	$$\E[ Y_{ij}] = \left(1-\frac{1}{m}\right) \cdot \gamma_{ij}^{\mathcal N\setminus \{i,j\}}(\one/m).$$
For $i = k$ the covariance of the link $u_i u_j$ with link $u_k u_l$ is given by (\ref{eqn:cov_a_HD}) using (\ref{eqn:state_weight_a_HD}) and the state coefficients
    %$$\alpha_{xyz}= \cdots$$
	%$$\begin{aligned}\alpha_{xyzw}(c) = \gamma_{xy}^{\mathcal N\setminus\{x,y\}}(\xi), \end{aligned}$$
	$$\begin{aligned}\alpha_{xyxw}(c) = \gamma_{xy}^{\mathcal N\setminus\{x,y,w\}}(c),% \ds \mbox{ where } c = [c_\nu]_{\nu \in \mathcal{N}\setminus\{i,j,k,l\}}.
	\end{aligned}$$
	 	where $c = [c_\nu]_{\nu \in \mathcal{N}\setminus\{i,j,l\}}.$
%where $\xi_{\nu}  = c_\nu$ if $\nu \ne k,w,$ $\xi_{k} = 1-\delta_{ik}$ and
%where $\xi_{\nu}  = c_\nu$ if $\nu \ne x,w$ and $\xi_{k}= \xi_w = 0.$

For $i \ne k,$  it is given by (\ref{eqn:cov_b_HD}) using (\ref{eqn:state_weight_a_HD}), (\ref{eqn:state_weight_b_HD}) and the state coefficients
	$$\alpha_{xyzw}(c') = \gamma_{xy}^{\mathcal N\setminus \{x,y,w\}}(\xi), \ds c' = [c_\nu']_{\nu \in \mathcal{N}\setminus\{i,j,k,l\}},$$%\; \mbox{ and } \;
	where $\xi = [\xi_\nu]_{\nu \in \mathcal N\setminus\{x,y,w\}},\,\xi_z =1,\, \xi_\nu = c'_\nu,\; \nu \ne z,$ and
	$$\beta_{xyzw}^{(d)}(c'')= \gamma_{xy}^{\mathcal N\setminus\{x,y,z\}}(\zeta), \ds c'' = [c_\nu'']_{\nu \in \mathcal{N}\setminus \{i,k\}},$$
 where  $\zeta = [\zeta_\nu]_{\nu \in \mathcal N\setminus\{x,y,z\}},\, \zeta_{\nu}  = \delta_{c''_\nu d}, d = 1,2.$
\end{cor}
\begin{proof}
This is a consequence of Theorem \ref{prp:slotCorrelationsHD} and   \cite{Nakagami12}. See 
\if\pubMode\IEEE
the technical report \cite{TechRep}
\else
Appendix  \ref{proof:cor_HD}
\fi
for details.
%We only give the main ideas; see
%\if\pubMode\IEEE
%    \cite{TechRep} 
%\else
    %Appendix \addRef{}
%\fi
%for a more elaborate version. If $P_{i\nu} \sim f_{ij}$ as in (\ref{eqn:naka_pdf}), then we have by \cite{Nakagami12} (using our notaion) 
%\begin{equation}\label{eqn:gamma_ij}\gamma_{ij}([\sigma_\nu]_{\nu\in \mathcal N\setminus\left\{ i,j \right\}}) = \Pr\left(\frac{P_{ij}}{N+\sum\limits_{\nu\ne i,j}^{}\Sigma_\nu P_{\nu j}} \ge \theta\right)\end{equation}
%for Bernoulli variables $\Sigma_\nu$ with parameters $\sigma_\nu$ such that $\Sigma_\nu,$ $P_{\nu, j},$ for $\nu \ne j,$ are mutually independent. 
%Hence, $\E X_{ij} = \Pr\left(\frac{P_{ij}}{N+\sum\limits_{\nu\ne i,j}^{}\Sigma_\nu P_{\nu j}} \ge \theta\right)$ for mutually indepentent Bernoulli variables $\Sigma_\nu$ with (\textit{call occurance}}) probability $1/m.$ 
%One can verify that $\Sigma_{\nu} := \delta_{S_i S_{\nu}}$ satisfies this property such that then $\E Y_{ij} = (1-1/m) \cdot \gamma_{ij}(\one/m).$% if we can show that 
%The second part of the claim then follows analogously by using only probabilites $\sigma_\nu = x_\nu \in \{0,1\}$ and from Theorem \ref{prp:slotCorrelationsHD}. 
	%%%$$\gamma_{ij}([\Sigma_\nu]_{\nu\in \mathcal N\setminus\left\{ i,j \right\}}) = \E X_{ij}$$
%for Bernoulli variables $\Sigma\nu$ with arbitrary call occurance probability. 
%We only have to use \cite{Nakagami12} to verify that  
%
\end{proof}  

In Fig.~\ref{fig:correlation} we show an example plot resulting from Corollary~\ref{cor:nakagamiHD} with Nakagami fading shape parameter $2$ and $2$ slots.  
The plot shows the correlation matrix for all possible communication links among $6$ nodes arranged on a $2\times 3$ grid (cf. Section \ref{sec:parameters}). 
%\begin{proof}
%See Appendix.	
%\end{proof} 



%From \cite{Nakagami12} it is known that under Nakagami-m fading the success probabilities are
	%\begin{equation}\label{eqn:Nakagami_success}\E X_{ij} = \cdots \end{equation}

\begin{figure}[t!]
	\centerline{\includegraphics[trim=400 80 400 40,clip, width = 0.35 \textwidth]{img/correlation_hinton.pdf}}
	%\includegraphics[trim=080 10 80 40,clip, width = 0.59 \textwidth]{img/correlation_hinton.pdf}
	\caption{\scriptsize Distribution of the correlation for a half-duplex example. White and black squares correspond to positive and negative correlation, respectively. A larger square means a larger correlation in modulus. At the largest ones on the diagonal the correlation is $+1.$ 
	The component (a) of Theorem \ref{prp:slotCorrelationsHD} corresponds to the white diagonal square blocks. \label{fig:correlation}}
\end{figure}  
%\subsection{MAC layer: slotted ALOHA model in the half duplex case}
\color{black}


==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/40_simulation.tex <==
\color{black}
\section{Application to Average Consensus}
\label{sec:application}
\subsection{Discrete probabilistic average consensus}
In the discrete, linear, first order probabilistic average consensus protocol \cite{Olfati-Saber2007}, \cite{Fagnani08}, \cite{Silva11}, a group of $n$ nodes periodically exchanges broadcast messages each containing a sender's dataset. 
For simplicity we assume all nodes have scalar, real valued data. It is an iterative random process whose goal is that all nodes agree on the same value in the limit with probability one. Further this value, the \df{agreement value}, should be close to the average of the initial data. Nonetheless, due to asymmetries in packet loss between outgoing and incoming transmissions, the agreement value will differ from the true average
%but lie within the convex hull of the initial values for suitable chosen gain parameter \addRef{belegen}.
which, however, shall not be our concern here.
%with the deviations from the average of the inital states here. 
Instead we focus on a probabilistic description of all nodes' deviation from the \textit{current} average at \textit{every} iteration. We measure this deviation in terms of the \textit{root mean square} (RMS) error (or \df{disagreement}) after $k\in \N$ iterations (or steps) which we now introduce: 
If the (random) vector $x_k = (x_k^{(1)}, ..., x_k^{(n)}) \in \R^n$ represents the nodes' states after $k$ consensus iterations having started from the deterministic initial state $x_0\in \R^n,$ then by $\sum_{i = 1 }^{n} \left( x_k^{(i)} - \frac{1}{n} x_k^T \one \right)^2$ a scalar random variable will be given which we shall denote by $\delta_k^2(x_0).$
	Divided by $\sqrt{n-1},$ the entity $\delta_k(x_0)$ is just the \textit{sample standard deviation} of the components $x_k^{(i)}, i = 1,\dots,n,$ explaining why it is also called \df{disagreement}. See e.g.\cite{Fagnani08} for further reading.
For any initial state $x_0$ the RMS error after $k$ steps is defined as $\sqrt{\E \delta_k^2(x_0)}.$ 

Finally, the \df{maximum root mean square} (mRMS) error is the RMS error for the worst possible choice of inital state inside the closed unit ball, $\max_{\n{x} \le 1}\sqrt{\E \delta_k^2(x)}.$ Note that the RMS error attains its maximum for \df{normalized} initial values, i.e. those on the unit sphere.

\subsection{Performance measure}
%We use the following slightly modified result from \cite{ICCCN19} to bound the root-mean-square (RMS) error of probabilistic average consensus after $k\in \N$ iterations (or steps) denoted by $\sqrt{\E \delta_k^2}.$
In this subsection we use slightly modified results from the literature to bound the mRMS error from above\cite{ICCCN19}  and below\cite{Ogura2013}. 
The mRMS error stochastically describes the consensus disagreement at the $k$-th step for the worst possible, step dependent choice of the initial state. It  constitutes a performance measure capable of well capturing the outage correlation effects.
%In \cite{ICCCN19} a Bernoulli model (BM) with symmetry and spatial uncorrelation was assumed. 
In \cite{ICCCN19} an uncorrelated half duplex Bernoulli model (UHBM) with symmetric packet losses was assumed. 
This assumption, however, does not affect the generality of the proof of the $k$-step estimates presented there, although some adaptions in notation are required.
%Since knowledge of the expectations of correlated Bernoulli variables is not sufficient to determine their joint distribution (as is already obvious for two variables), we need to adapt the notation in the theorem below (e.g. from $r_2(L, \varepsilon)$ to $r_2([Y_{ij}], \varepsilon)).$

To quantify the impact of outage correlation on consensus, let us introduce $n^2-n$ uncorrelated Bernoulli variables $Z_{ij}, i \ne j,$ rendering an asymmetric %(uncorrelated, asymmetric) BM
UHBM having the property\footnote{The symmetric UHBM of \cite{ICCCN19} has the alternative property $\E Z_{ij} = \E Z_{ji} = \E (Y_{ij} + Y_{ji})/2$ which we do not use here.}
	$\E [Z_{ij}] = \E [Y_{ij}],$
where $Y_{ij}$ are defined in section IV.
In particular $\cov(Z_{ij}, Z_{kl})=0,$ for $i \ne j, k \ne l$ and $(i,j) \ne (k,l).$ 


To apply the UHBM and our correlated half-duplex Bernoulli model (CHBM) in the consensus context, we need to link the uncorrelated variables $Z = (Z_{ij})_{i\ne j}$ and their correlated counterparts $Y = (Y_{ij})_{i\ne j}$ to so called \textit{Laplacian} valued random matrices $L^{Z}$ and $L^{Y}$ respectively: For any ensemble of Bernoulli variables $W = (W_{ij}),\, 1 \le i,j \le n, i \ne j,$ define $L^W= (\ell_{ij}^W)$ by 
	%$$\ds \ell_{ii}^W = \sum_{\substack{k=1\\k\ne i}}^{n} \ell_{ik}^W\ds \mbox{ and }\ell_{ij}^W = -W_{ij}, \ds 1 \le i,j \le n, i \ne j,$$
	$$ \ell_{ij}^W = \left\{ \begin{aligned} &\sum_{\substack{k=1\\k\ne i}}^{n} W_{ki}, \ds &\mbox{ if } i = j,\\
		&-W_{ji}, \ds &\mbox{ if  } i \ne j  .\end{aligned}\right.$$
Note that for any $\varepsilon >0$ and any sequence $W^{(1)}, W^{(2)}, \dots$ of realizations\footnote{More precisely, $(W^{(1)}, W^{(2)},\ldots)$ is supposed to be a random sample with $W^{(k)}\stackrel{\text d}{=} W,\; k\in\N$, where $\stackrel{\text d}{=}$ means equality in distribution.}  of $W$ the discrete consensus protocol \cite{Olfati-Saber2007}, \cite{Silva11}, (also cf. \cite{ICCCN19}) is then given by the matrix iteration
	$$ x_{k+1} = (I_n - \varepsilon \cdot L^{W^{(k)}})\cdot  x_k,$$
	provided the values $W_{ij} = 0, 1$ are interpreted as unsuccessful/successful links $u_i u_j,$ i.e. $W$ represents the offdiagonal entries of a (transposed) adjacency matrix of an (in general undirected) graph (without loops); $x_0 \in\R^n$ is some arbitrary initial value. We call the number $\varepsilon$ \df{(discrete) gain}.
	We assume the realizations $W^{(1)}, W^{(2)}, \dots$ to be mutually independent, which reflects the IBF assumption. Note that from the communication perspective, this constitutes a sequence of frames; the slots play only an implicit role causing the correlation within any of the $W^{(k)}$'s.
Now let
	$$R^W(\varepsilon) :=  (\Pi \otimes \Pi) \cdot [(I_n- \varepsilon \E L^W)\otimes(I_n- \varepsilon \E L^W) + \varepsilon^2 C^W] $$
where the matrix $C^W\in \R^{n^2 \times n^2}$ is given in terms of its components $C^W_{IJ} = \cov(\ell_{ij}^W, \ell_{kl}^W),$ for $I = (n-1)\cdot i +k , J = (n-1)\cdot j + l, \ds i,j,k,l = 1 ,\dots, n.$
Since the covariance is a bilinear form, these components can be easily determined in terms of $W.$ E.g. for $W=Y$ and $i = j$ and $k\ne l$ we have $\cov(\ell_{ij}^Y, \ell_{kl}^Y) = -\sum_{\substack{\nu = 1\\ \nu \ne i}}^{n} \cov(Y_{\nu i}, Y_{lk}).$ Similarly, $\E [L^W]$ can be evaluated.
Finally, we can define the $L^2$-joint spectral \cite{Ogura2013} and numerical radius \cite{ICCCN19}, respectively ,
	$$r_2(W,\varepsilon) := \sqrt{\varrho(R^W(\varepsilon))} \mbox{ and } w_2(W, \varepsilon) := \sqrt{w(R^W(\varepsilon))},$$
where $\varrho(\,\cdot\,)$ denotes the spectral radius (i.e. the largest modulus of all eigenvalues) and $w(\,\cdot\,)$ denotes the numerical radius, e.g. \cite{He1997a}, of a matrix. 

The following theorem introduces an upper and a lower bound for the latter of which there always exists a normalized initial state $\hat x$ (i.e. $\n{\hat x} = 1)$ such that $\sqrt{\E \delta_k^2(\hat x)}$ exceeds or attains the lower bound. On the other hand, for \textit{any} normalized initial state $x$ %we have that $\E \delta_k^2(x)$ stays below or attains the upper bound.
the upper bound dominates $\sqrt{\E \delta_k^2(x)}.$

\begin{thm}[cf. \cite{ICCCN19} and e.g. \cite{Ogura2013}]\label{thm:bounds}
Let $W = Y,Z$ represent the %correlated model or the (uncorrelated) Bernoulli model. 
CHBM or the UHBM.
Then the mRMS disagreement after $k$ iterations is bounded as follows:
$$\frac{r_2^k(W, \varepsilon)}{\sqrt n} \le \max_{\n{x} \le 1}\sqrt{\E \delta_k^2(x)} \le \sqrt{2\sqrt{n-1}}\cdot w_2^k(W, \varepsilon).$$
\end{thm} 
\begin{proof}
	The left-hand inequality follows from the infimum property of $r_2$, e.g.\cite[Lem. 2.7]{Ogura2013}), the right-hand one from \cite{ICCCN19} up to a factor of %$\sqrt{\frac{n-1}{n}}.$ See \AddRef{TechRep}
	$\sqrt[4]{(n-1)/n}.$ See 
	\if\pubMode\IEEE
    	\cite{TechRep}
    \else
    Appendix \ref{prf:thm:bounds}
    \fi
    for details.
\end{proof}

%It now seems natural to define  lower and upper performance bounds after $k$ steps

In analogy to the geometric mean we now define the following lower and upper performance bounds for the \df{average per step}  mRMS error, $\max_{\n{x} \le 1}\sqrt[2k]{\E \delta_k^2(x)}:$ %after $k$ steps:
%$$ \frac{r_2(W,\varepsilon)}{\sqrt[2k]{n}} \mbox{ and } (2 \sqrt{n-1} )^{1/2k} \cdot w_2(W,\varepsilon) $$
\begin{equation}\label{eqn:bounds}\text{lb}(\varepsilon)= \frac{r_2(W,\varepsilon)}{\sqrt[2k]{n}}\; \mbox{ and }\;
\text{ub}(\varepsilon) = \sqrt[2k]{2 \sqrt{n-1}} \cdot w_2(W,\varepsilon),\end{equation}
%respectively,
where $\text{lb}(\varepsilon) =\text{lb}(\varepsilon;k,W)$ and $\text{lb}(\varepsilon) = \text{lb}(\varepsilon; k,W).$ 
\begin{rem}
\label{rem:thm_bounds}
\begin{rom}
%Note that 
\item
Asymptotically, the lower bound is tight since $r_2(W,\varepsilon) = \lim\limits_{k\sra \infty}\max_{\n{x} \le 1}\sqrt[2k]{\E \delta_k^2(x)},$
\if\pubMode\IEEE
cf.\cite{TechRep}.
\else
(cf. Appendix \ref{sec:appendix_additional}).
\fi
\item The number of steps $k$ required to obtain a prescribed precision
increases only logarithmically with the number of nodes $n$ (apart from the spread of $r_2$ and $w_2$). %Note further  that

\item The upper bound used in \cite{Silva11} is simply the squared mRMS disagreement for the first step ($k=1$),  \if\pubMode\IEEE
cf. \cite{TechRep}.
\else
cf. Appendix \ref{sec:appendix_additional}.
\fi
\end{rom}
\end{rem}

%In Fig. \ref{fig:performance_bounds} we use $k = \numberOfSteps.$ The 
%\comment{Add link to slot model}



\subsection{Exemplary effects for a selected deployment and parameters}
\label{sec:parameters}
We adopt network parameters similar to the IEEE 802.11p standard: A carrier frequency of 5.9 GHz and a bandwidth $B$ of 10 MHz. We choose a reference bitrate $R_0$ of 40\% of the 802.11p maximum bitrate of 27 Mbit/s. To obtain comparable consensus performance results, we let the beacon time interval be constant in terms of slots, more precisely we set $R$ according to the number of slots $m$ in use: $R = m \cdot R_0.$ The threshold $\theta$ is then computed according to Shannon capacity formula: $\theta = 2^{R/B}-1.$ For $m=1$ we obtain $\theta = 2.23$ such that the requirement $\theta \ge 1$ is always fulfilled. The thermal noise parameter $N$ is obtained from the Boltzmann constant $k_B$ at a reference temperature $T$ of 293K: $N = B\cdot k_B \cdot T.$

Our nodes are deployed on a regular $2\times 3$ grid having a horizontal and vertical distance of 1500m between neighbors, a common transmit power of 500 mW, a common varying Nakagami shape paramter $m_i = m_S, i = 1 , \ldots, n,$ and a path loss coefficient of 2.0.

Figures~\ref{fig:performance_bounds_by_slots} and \ref{fig:performance_bounds_by_shape} show
the consensus performance (\ref{eqn:bounds}) over the gain parameter which is scaled in terms of the \df{minimizer} $\varepsilon$ of the \df{essential spectral radius} $\varrho(\Pi- \varepsilon \E [L^W]),$  e.g. \cite{ICCCN19}.%, also see
%\if\pubMode\IEEE
%    \cite{TechRep}.
%\else
%    \addRef{}.
%\fi
The minimizer, denoted by $\varepsilon_\varrho(m,m_S),$ depends on the number of slots and the shape parameter unitilized, but is the same for the correlated and uncorrelated model, $W = Y,Z.$ 
%We apply the performance bounds (\ref{eqn:bounds}) and
We set $k$ to \numberOfSteps\ steps.
%Note that for the given node positions and for the network settings chosen, the figures describe the consensus in our model used almost completely.

 
In Figure~\ref{fig:performance_bounds_by_slots} the number of slots is varied, in Figure~\ref{fig:performance_bounds_by_shape} the shape parameter.
%In Figure  \figurePerformanceBoundsByShape\ the graphs are denser, so we desist from plotting both upper and lower bound. Instead we chose the mean $\frac{\text{lb}+\text{ub}}{2}(\varepsilon).$ The difference between both bounds is similar as in Figure \figurePerformanceBoundsBySlots.
We observe two effects. (i) In both figures the correlated model shows significantly better performance and also different locations of the minimizing gain setting $\varepsilon$ (the minimizer of the correlated model is closer to $\varepsilon_\varrho$). (ii) Remarkably, in Figure~\ref{fig:performance_bounds_by_shape} the order of the curves in terms of performance is inverted: Curves
 with lower shape parameter perform better in the uncorrelated model while they perform worse in the correlated one. 
%While we suspect that effect (i) holds quite generally
%While we expect effect (i) to hold quite generally
While we observed effect (i) for various parameter settings (Figure~\ref{fig:performance_bounds_by_slots}, $m=6$ constitutes a borderline case), effect (ii) is rather unusual.
% for the purpose of exposition.

%\begin{figure}[t!]
	%\centerline{\includegraphics[trim=080 20 80 50,clip, width = 0.55 \textwidth]{img/deployment.pdf}}
	%\caption{\scriptsize  Node deployment}
%\end{figure}

%\begin{figure}[t!]
%	\label{fig:performance_bounds}
%	\centerline{\includegraphics[trim=080 5 80 40,clip, width = 0.49 \textwidth]{img/w2.pdf}}
%	\caption{Comparison of exact performance (cor. - solid curve - vs. uncor. - dashed curve -) after \numberOfSteps consensus iterations, here for ?? slots and shape parameter ??. The true \numberOfSteps step performance lies within the shaped areas.}
%\end{figure}      

\begin{figure}[t!]
	%\centerline{\includegraphics[trim=080 10 80 40,clip, width = 0.49 \textwidth]{img/half-duplex.pdf}}
	%Performance by slots \label{fig:performance_bounds_by_slots}
	
	\centering
	\subfloat[\label{fig:performance_bounds_by_slots}Performance for different frame lengths $m.$ ]{\includegraphics[trim=080 5 80 40,clip, width = 0.49 \textwidth]{img/half-duplex_r2w2.pdf}}\hfill
	\subfloat[\label{fig:performance_bounds_by_shape}Performance for different Nakagami shape parameters $m_S.$]{\includegraphics[trim=080 5 80 40,clip, width = 0.49 \textwidth]{img/gradient2.pdf}}\hfill 

\caption{\scriptsize Comparison of the consensus performance for uncorrelated ($W=Z,$ dashed curves) and correlated model ($W=Y,$ solid curves) in terms of the upper and lower bounds (\ref{eqn:bounds}) for $k = \numberOfSteps$ steps. On the abscissa we lay off the gain parameter scaled by the optimal essential spectral radius for the pair $(m,m_S),$ on the ordinate the dimensionless bounds (\ref{eqn:bounds}). Smaller values correspond to better performance, a value below (above) 1 for \textit{both} bounds implies (in-)stability in the exponential mean square sense \cite{Ogura2013}. Further, at a scope of $k$ steps the average per step mRMS error
%, $\max_{\n{x} \le 1}\sqrt[2k]{\E \delta_k^2(x)},$
lies within the colored regions. In Figure \ref{fig:performance_bounds_by_slots} the shape parameter $m_S$ is set to $1$ (Rayleigh fading) while the number of slots per frame $m$ varies. In Figure \ref{fig:performance_bounds_by_shape} the frame length $m$ is fixed to $3$ while the shape parameter $m_S$ varies.}
%    \caption{\scriptsize $r_2$-performance in the half-duplex case with Rayleigh fading. Similar details apply as in Fig. 1. The correlation is stronger in this case which is also reflected by the difference of the $r_2$ performances of correlated and uncorrelated model.\\ The $r_2$-performance is a dimensionless entity describing the exponential decay of the root mean square error (the lesser the better), here for the full-duplex case with Rayleigh fading. The dashed curves represent the uncorrelated model while the solid ones represent the correlated model for varying numbers of slots $m.$ On the abzissa the (discrete) gain is shown in units of the optimal gain in terms of the algebraic connectivity $\lambda_2.$ Thus it depends on the number $m$ of slots utilized.  E.g. using the optimal $\varepsilon$ in terms of $\lambda_2$ leads to an unstable system for $m=2$ in the uncorrelated model and to a stable system if correlations are taken into account (blue dashed resp. solid curve at $\varepsilon = \varepsilon_{\lambda_2}$).}
\end{figure}
 
  

%\begin{figure}[t!]
	%\label{fig:performance_bounds_by_shape}
	%\centerline{\includegraphics[trim=080 5 80 40,clip, width = 0.49 %\textwidth]{img/gradient2.pdf}}
	%\caption{\scriptsize vermutlich $alpha \ne 2.0 $ replace $r_2$ with %$\frac{\text{lb}+\text{ub}}{2}(\;\cdot\;; \numberOfSteps, W)$}
%\end{figure}    


%\caption{\scriptsize  } 

==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/50_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
We have derived closed form expressions for the outage/success correlation in a framed slotted ALOHA scheme under the Nakagami fast fading model for fixed relative node positions.
%The result extends the work \cite{Nakagami12} and \cite{ICCCN19}. The correlation is due to the random choice of slots. 
The found expressions enable a thorough performance analysis of distributed control applications in wireless networks for which we provide bounds in an appropriate form.

Although inaccurate compared to the correlated model, the uncorrelated one %, although inaccurate,
could still serve %suited/adequate to provide worst case 
as rough but simpler structured bound for the control performance. How far it is sufficient to use the simpler bound requires a broader study.
%is sufficient a broader study is required.

Our method can in principle be carried over to related slotted ALOHA protocols, e.g. spatial and opportunistic spatial ALOHA \cite{Baccelli2009a}. %\cite{Ishii2017}.
Apart from the broadcast case, an application in interference cancellation\cite{Clazzer2017} is also thinkable.

%\textbf{Vielleicht noch folgende Argumentation ins Fazit aufnehmen:}
%\begin{itemize}
%    \item Rayleigh fading und unkorreliertes Modell eignen sich als %worst/bad case Abschaetzung
%    \item oder zumindest als future work genauer untersuchen, ob sich das wirklich eignet
%    \item Also: our work suggests that the uncorrelated Bernoulli model, although inaccurate, may be suited/adequate under Rayleigh fading to provide worst case performance estimates which is of interest by virtue of its simplicity and ought to be clarified in further studies. 
%    \item Gleichzeitig auch vielleicht auf $\lim_{n \rightarrow \infty}$ eingehen: Future work!
%    \item Bachelor-Arbeit? (mal großflaechig den Parameterraum absuchen! Neues Modell? Kombination aus 
%     $\rho$ und unkorreliertem Bernoulli model
%\end{itemize}
%and reveal modeling errors of uncorrelated Bernoulli models.


==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/80_references.tex <==

%\newpage
%\ 
%\newpage

\bibliography{bibfile}{}
\bibliographystyle{plain}


==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/990_intro_alt.tex <==
\begin{abstract}
ADD STUFF

\begin{itemize}
	\item As the average consensus protocol is linear it 
	\item Closed from expressions for slotted ALOHA, general case and Nakagami fading
\end{itemize}



\begin{IEEEkeywords}
L2 joint spectral radius, L2 joint numerical radius, First Order Consensus, Nakagami fading, convergence speed.
\end{IEEEkeywords}

\end{abstract}

\begin{td}
	\begin{itemize}
		\item Voll-Duplex Modell ist gut, um Konsens-Effekte auch fuer kleine Knotenzahlen studieren zu koennen
		\item $ \leadsto \E Y_{ij}Y_{kl}$ berichtigen
		\item 

	\end{itemize}<++>
\end{td}<++>


\textbf{Timetable:}\\
\textbf{By Monday, Feb 3:}
\begin{itemize}
    \item Thorough differentiation from the Haenggi correlation model used in the PPP.
    \item Related work on Nakagami-Fading and outage proabilities in finite networks  $\checkmark$
    \item Proofs of the correlation statements $\checkmark$
    \item Clean and complete statements of the Correlation Proposition and the connection with the ICCCN paper.
    
    
\end{itemize}

\textbf{ By Monday, Feb 10:}
\begin{itemize}
    \item Finalize the Introduction and Related Work according to status quo
    \item General communication focus without particularizing to consensus: 
    \begin{itemize}
        \item Discuss the Simulation/Sampling of the correlation in comparison to the exact formula. 
        \item Provide relative errors in an overview for $n \le 20$ nodes, e.g. n= 6, 10, 15, 20.
        \item Discuss tendencies and possible effects that might have to be considered when using the simulation as an approximation of the formula for $n > 20$ nodes.
    
    
    \end{itemize}
    
    \item Consensus:
        \begin{itemize}
            \item Description of the consensus plots for at least one node deployment for few plausible choices of slots.
            \item Optional: discuss the n=30 case
    \end{itemize}
    
\end{itemize}

    
    
    

\begin{td}
	\item add item Add Lyapunow exponent
\end{td}


\begin{itemize}
	\item Related work: What are the problems/benefits of $r_2,$ versus the lyaponow exp.
	\item Related work: rare events
	\item Related work: Fading!!
	\item Related work: Correlation!!
\end{itemize}


\section{Introduction}
Blabla

%The general direction of research aimed by this work is to quantify the influence of correlations due to media access control schemes on distributed average consensus in a wireless scenario. 
The goal of this work is to quantify the correlations due to media access control schemes for wireless sensor nets (WSN) and for snapshots of ad-hoc-Networks. The results of this work can
be immediately applied to the analysis of distributed cooperative control protocols, such as probabilitstic average consensus \addRef.
Example applications consist of weather measurements (WSN) \addRef and formation control (cooperative control) \addRef.



Concrete, we consider a deployment of $n$ nodes moving in the plane which perform first order, probabilistic average consensus \addRef. As quality measure we use a probabilistic entity describing the instantaneous\footnote{Instantaneous means here that in the analysis we consider snapshots of the nodes' positions. However, the performance of trajectories can be bounded stepwise, e.g. by the measure $\n{\tilde R}$ of \cite{ICCCN19} which is closely related to $r_2.$} exponential decay of the mean squared error/disagreement: the $L^2$-joint spectral radius \addRef or generalized joint spectral radius , which we call $r_2$ \addRef. Since we aim at formal treatment, we employ slotted ALOHA as simple media access scheme for broadcast communication\addRef. Here we have also additional consequences in mind which regard the IEEE 802.11p protocol since the latter can behave like slotted ALOHA at high densities \cite{Baccelli13}. 

The central question of this paper is how the correlation due to each node's choice of the transmission window affects the consensus performance in terms of $r_2,$ compared to a model where packet reception along each link is mutually independent. We have investigated the latter situation in our earlier work \cite{ICCCN19} where we incorporated the SINR physical layer model - recommended in \cite{Iyer09} - with Rayleigh fading and established closed form expressions for successful transmission for each link. In this work we will generalize to Nakagami fading and derive closed form expressions for the covariance between links. These expressions are then fed into the matrix $R$ which is related to $r_2$ by $r_2 = \varrho(R)$ \cite{ICCCN19}, where $\varrho(\cdot)$ denotes the spectral radius of a matrix. 

A second aspect arises when acutally verifying the theorerial findings by simulations of the consensus scenarios.  As we have briefly observed in \cite{ACC18}, rare events of ``bad behavior'' may have large impact on $r_2$ since it is a mean square measure. 
%It would of course be ideal to additionally consider the $L^{1}$-joint spectral radius \addRef characterizing the mean disagreement/error, since it assigns a smaller weight to badly behaving rare events. 
In general, the $L^p$-joint spectral radius (in short $r_p$), $p\ge 1$, characterizes exponential stabiltiy in terms of the mean of the disagreement raised to the $p$-th power ($p$-th mean stability) \addRef{Ogura14}.
Thus, it would of course be ideal to additionally consider $r_1$ \addRef, since it assigns a smaller weight to badly behaving rare events. However, $r_p$ can be computed easily only if $p$ is either even or the random measures representing the communication satisfy a certain geometric property on convex cones \addRef{Protasov} which is not the case for $r_1$ since it would then simply coincide with the essential spectral radius \addRef{Ogura14 oder LA}.

Moreover, a computation of $r_1$ cannot constitute a full solution since the impact of rare events is already present for first mean stability, which is considered in \cite{Moura13}. There, these events are worst case paths with sub-exponential decay in disagreement and are called \textit{large deviations} stemming from the Large Deviation Theory, e.g.\addRef. The authors found that sub-exponential paths do not exist if the communication graph is connected at all instances. The latter is, however, not the case in our modelling scenario. Thus, empirical measurements of the squared disagreement cannot solely be trusted as they can suggest faster convergence than there actually is - a fact that we observe in our simulations for mean square convergence. \comment{Vergleich Bernoulli Simulation, was ist besser?}

%The question comes up why this is the case. To investigate 
To investigate why this is the case 
\begin{itemize}
	\item 2-fold: Im statischen Fall tritt es schon auf \dots
\end{itemize}

It sheds some light on the fact

\begin{itemize}
	\item ICCCN-Paper stellt $k$-Schritt-Abschätzungen bereit.
\end{itemize}


 and investigate 
\textbf{Outline}
\begin{itemize}
	\item iid fading channels
	\item still correlation in slotted aloha $[RW]$
	\item static node setting, no PPP
	\item based on our work \cite{ICCCN19}

	\item SINR \textbf{Further, we feel that an SINR-based model is the minimum level of detail that should be employed to model wireless channel interference} \cite{Iyer09}

\end{itemize}  


==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/9999_aussortiert.tex <==
\subsection{Sketch of Proposition XYZ's proof}

\qed
% END OF PROOF 2
\newpage

\subsection{Slotted CSMA and slot picking ALOHA}
Here, we briefly recapitulate the abstraction of the IEEE 802.11p protocol introduced in \cite{Baccelli13} called slotted CSMA and the corresponding slotted ALOHA model we term slot picking.

Assume a broadcast scenario where all nodes have to transmit a packet every $\tau$ ms. This beacon time interval is called a \df{frame} which is divided into $K$ slots. A node may come with a fixed (time) offset $m = 0, \dots, K-1,$
thus always transmitting 

making it a node of class $m,$ Moreover, each slot is divided into an interframe space and a number $CW$ of subsequent backoff slots followed by the packet transmission duration. 

The beacon time interval is divided into $m$ slots of equal length and the network is dominated by nodes whose \df{backoff counter} is $0$ in the beginning of a slot, i.e. it will send immediately after IFS.


\subsection{Removed}
Motivation: Usual first order continuous time dynamics consensus prototocol with time varying Laplacian $L = L(t)$:
    $$\dot x  = - L x $$
After differentiation, we have
    $$\ddot x = - L \dot x - \dot L x $$
To reduce the blow-up events, let us introduce a velocity dependent damping term with parameter $\sigma:$
$$\ddot x = - L \dot x - \dot L x - \sigma \dot x,$$
or
%$$\ddot x = - (L + \sigma I) \dot x - \frac{\mbox{d}}{\mbox {d} t} (L + I) x  = - \frac{\mbox{d} }{\mbox{d}t}(L + I) x$$
$$\ddot x = - \frac{\mbox{d} }{\mbox{d}t}(L + I) x.$$
After integration (and neglecting the integration constant) we arrive at
$$\dot x = - L^{\sigma}x := -(L + \sigma I) x$$
which translates to the following disagreement dynamics:
    $$\dot \delta = - (L + \sigma \Pi) \delta.$$
Letting $P^\sigma = I - \varepsilon L^\sigma, \varepsilon> 0,$ we have 
	$$ P^\sigma \one = (1-\varepsilon \sigma) \one $$
and 
	$$ P^\sigma $$

When discretizing just substitute L with (L + sigma * id). Thats it. (I know that this does not preserve the average and that 1 is no right-eigenvalue of 1|, this can be fixed e.g. by using sigma * Projection-matrix instead of sigma* id which again has the disadvantage of not having a distributed implementation, but I merely need this as a theoretical construct for analysis and as argument to support the measurements).

I know that having a damping is quite usual in double-integrator systems, e.g. eq (7) [2.pdf].

\subsection{Removed}
 \begin{prp}[\cite{ICCCN19}]
\label{prp:ICCCNprobabilites}
The probability for successful transmission from node $u_i$ to node $u_j,$ while all nodes are constantly competing for slots, is given by the formula
%$$\begin{aligned}p_{ij}(k) &= (1-\frac{1}{k}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{k (\theta + \mu_{mj} / \mu_{ij}})\right)\\
%	&=\frac{k-1}{k^{n-1}} \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(k- \frac{\theta}{\theta + \mu_{mj} / \mu_{ij}}\right)\\ &=: \sum_{m=0}^{n-1}a_{ijm}k^{-m} \end{aligned}$$
%\begin{equation}\label{eqn:p_ij}p_{ij}(m) &= (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{m (\theta + \mu_{mj} / \mu_{ij})}}\right).\end{equation}
\begin{equation}\label{eqn:p_ij}p_{ij}(m) = (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{k\ne i,j} \left(1- \frac{\theta}{m (\theta + \mu_{kj} / \mu_{ij})}\right).\end{equation}
\end{prp} 


 \begin{itemize}
	\item If $L$ is not symmetric, we do not even have $\E x_{\infty} = \frac{1}{n} \one x_0.$
	\item Performance measures: $r2$, Lyapunov exponent
	\item In $r_2$ large, unlikely deviations contribute a lot. $r_1$ cannot be evaluated easily.
	\item Related work criterium in terms of $n$ and $?$: When is $r_2^k$ close to $\E \n{\Pi P_k \dots P_1}^2?$
	\item They say that one should use the $r_2$ if $n \gg 1$ and otherwise the Lyapunov exponent \comment{verify}.
	\item Other related work: symmetric instances, they measure rare subexponential paths. \cite{Moura13}
	\item However, we think neglecting these catastrophic events, which lead to the deviation of the actual squared disagreement from the expected squared disagreement, is not always the best. 
	      Because of the linear nature of the consensus protocol, agents will in practice not be able to follow the protocol once the physical limitations are reached. In simulations one
 	      can model this behavior for instance by simply adding a maximum velocity and thus a maximum possible displacement per time step. If the disagreement is small, bounding the displacement
	      has no effect. If it is large, the displacement will capped. This protocol is, however, no longer linear. To add 
\end{itemize} 


 \textbf{Timetable:}\\
\textbf{By Monday, Feb 3:}
\begin{itemize}
    \item Thorough differentiation from the Haenggi correlation model used in the PPP.
    \item Related work on Nakagami-Fading and outage proabilities in finite networks  $\checkmark$
    \item Proofs of the correlation statements $\checkmark$
    \item Clean and complete statements of the Correlation Proposition and the connection with the ICCCN paper.
    
    
\end{itemize}

\textbf{ By Monday, Feb 10:}
\begin{itemize}
    \item Finalize the Introduction and Related Work according to status quo
    \item General communication focus without particularizing to consensus: 
    \begin{itemize}
        \item Discuss the Simulation/Sampling of the correlation in comparison to the exact formula. 
        \item Provide relative errors in an overview for $n \le 20$ nodes, e.g. n= 6, 10, 15, 20.
        \item Discuss tendencies and possible effects that might have to be considered when using the simulation as an approximation of the formula for $n > 20$ nodes.
    
    
    \end{itemize}
    
    \item Consensus:
        \begin{itemize}
            \item Description of the consensus plots for at least one node deployment for few plausible choices of slots.
            \item Optional: discuss the n=30 case
    \end{itemize}
    
\end{itemize}

    
\subsection{Aussortiert}
  \begin{itemize}
	\item Managing Interference Correlation Through Random Medium Access \cite{Haenggi14}: Correlation between different slots (we consider all of them as a whole) and PPP, ALOHA and FHMA
	\item Hanggi: Correlation between different receivers in PPP, we: correlation between all links in a fixed scenario 
	
	\item still correlation in slotted aloha $[RW]$
	\item Consensus algorithms over fading channels \cite{Chan10}: Fading is not fast fading; just complex circularly symmetric noise with zero mean and variance $1.$ (And: Example graph for slotted ALOHA: convergence time over transmission probability.)
	\item stochastic geometry, interference, non-slotted ALOHA  \cite{Muhle14}
	\item Convergence Speed of the Consensus Algorithm With Interference and Sparse Long-Range Connectivity

\end{itemize} 
\begin{itemize}
	\item Frage: Wie haengen bei uns Kovarianz und Korrelation zusammen
	\item 
\end{itemize}

\begin{itemize}
%	\item Correlation, \cite{Haenggi14}, \cite{Benef04} \comment{(sehr aehnlicher Titel!!)}
	\item 
	\item Consensus \cite{Silva11}, \cite{Fagnani08},  \cite{ICCCN19}, %\cite{Moura13},

	%\item Convergence measures 
\end{itemize}


\begin{itemize}
	\item convergence speed in deterministic average consensus is directly linked to the algebraic connectivity which makes it an ideal prototye application
\end{itemize}
\begin{itemize}
	\item iid fading channels
	\item static node setting, no PPP
	\item SINR \textbf{Further, we feel that an SINR-based model is the minimum level of detail that should be employed to model wireless channel interference} \cite{Iyer09}
\end{itemize}  

\textbf{How is the paper organized?!}   

\begin{td}
	\begin{itemize}
		\item $ \leadsto \E Y_{ij}Y_{kl}$ berichtigen
		\item Mean-square Analyse weit verbreitet. Allerdings schrecken bei $r2$ alle vor den großen Systemen zurück.

	\end{itemize}
\end{td}
 \section{Intro}
 \section{Introduction}
During the past decades wireless sensor networks (WSN) and distributed multiagent systems have attained a lot of research interest in both communication and control community.
The goal of this work is to quantify the outage correlations due to media access control schemes for finite wireless sensor nets (WSN) and for snapshots of multi agent systems. %The results of this work can be immediately applied to the analysis of distributed cooperative control protocols, such as probabilitstic average consensus \addRef{}.
%Example applications consist of weather measurements (WSN) \addRef{} and formation control (cooperative control) \addRef{}.
 
While there is much work on the specifics of either side, few analytical papers consider a unifying approach where the impact of real network phenomenons is measured  directly in terms of distributed control performance as is done in our application.  
The effect of channel correlation has been investigated from a information theoretical point of view \cite{Benef04} as well as average over stochastic point processes \addRef{}. The effect of narrow band fast fading is considered mostly in a point process setting (\comment{belegen}) except for instance in \cite{Nakagami12} which we build upon. 

\addRef{PIMRC18: A pair of closely spaced receivers will receive similar interference even if the interference is received over fading channels that are decorrelated in space and time. This is because the loca- tion of interferers are a common source of randomness, even if the fading channels that they are observed over are not common. \\To the best of our knowledge, this paper is the first attempt to capture both finite network effects and interference correlation within a single unified analysis} 

On the other hand, when consensus is studied from the control perspective,
\addRef{Multi-agent Formation Control with Maintaining and Controlling Network Connectivity und das mit der konvexen Laplacematrix; oversimplified}

Although correlation is beneficial for MIMO capacity\cite{Benef04}, it is often considered bad in media access control (MAC), e.g. (temporal) correlation in different slots has negative impact on retransmissions \cite{Ganti2009}. We analyze outage correlation in the slotted ALOHA media access protocol and measure the effects on distributed schemes in terms of the performance of the average consensus protocol where we observe a benefitial impact for the most part. The applications we have in mind all require broadcast transmission such that Request To Send/Clear To Send (RTS/CTS) mechanisms cannot be applied. With increasing node density also carrier sensing becomes less and less beneficial, e.g. the IEEE 802.11p protocol can behave like slotted ALOHA\cite{Baccelli13}. 

Finally, the simplicity of slotted ALOHA allows for exact theoretical analysis (previous work considers mosty PPP theory \cite{Haenggi14}, \cite{Kim2019}, \cite{Talarico2018}).
Example applications consist of formation control, flocking (cf. the references in \cite{Olfati-Saber2004} and \addRef{ControlPaper}) or purely computational tasks like Gram-Schmidt orthogonalization which can be used to determine the network size \cite{Sluciak2013} or for further signal processing tasks, e.g. \cite{Sluciak2016}.
We make the observation that correlation is beneficial here compare to an (uncorrelated) Bernoulli process with the same (inhomogenous) outage probabilities.

We observe further that the outage correlation consists of two different components, a strong, positively correlated one and a weak, negatively correlated one (Fig. \ref{fig:correlation}??). The strong one shows up between a sender and all recipients and decreases as spatial distance gets bigger. The weak one affects the remaining links.

As application we consider a deployment of $n$ nodes moving in the plane which perform first order, probabilistic average consensus \cite{Olfati-Saber2004}, \cite{Fagnani08}, \cite{Silva11}. As quality measure we use a probabilistic entity describing the instantaneous\footnote{Instantaneous means here that in the analysis we consider snapshots of the nodes' positions.} %However, the performance of trajectories can be bounded stepwise, e.g. by the measure $\n{\tilde R}$ of \cite{ICCCN19} which is closely related to $r_2.$}
exponential decay of the mean squared error/disagreement: the $L^2$-joint spectral radius \cite{Ogura2013} or generalized joint spectral radius, which we call $r_2$ and which allows for exact characterization of (exponential) mean square stability.
Since we aim at formal treatment, we employ a slotted ALOHA variant as simple media access scheme for broadcast communication\addRef{}. %Here we have also additional consequences in mind which regard the IEEE 802.11p protocol since the latter can behave like slotted ALOHA at high densities \cite{Baccelli13}. 

This paper provides the methods to judge how the correlation due to each node's choice of the transmission slot affects the consensus performance in terms of $r_2,$ compared to a model where packet reception along each link is mutually independent. We have investigated the latter situation in our earlier work \cite{ICCCN19} where we incorporated the SINR physical layer model with Rayleigh fading and established closed form expressions for successful transmission for each link. In this work we will generalize to Nakagami fading and derive closed form expressions for the covariance between links. Also we adapt the stepwise bound $w_2$ of \cite{ICCCN19} to the correlated setting. 

An Application to consensus already shows examples of ``correlation network effects.'' For instance, we have found a situation such that when - loosly speakeing - varying the two parameters discrete gain and Nakagami shape parameter, the (sub-)gradient is by trend mirrored at the gain axis when switching from correlated to uncorrelated model.

In the following two sections we discuss related work, the overall notation, and the background needed to discuss the physical layer model. In section \ref{sec:corr} we introduce our MAC layer abstraction for slotted ALOHA and derive expectation and covariance of successful transmissions along links. Section \ref{sec:application} deals with an application of our result to a control theoretic multi agent system performing average consensus. Finally, the conclusion summarizes the paper and points out ideas for future work.

%We provide covariances for two modes \comment{Da fliegt full-duplex wohl raus}: Full and half-duplex. In full duplex we allow sending nodes to receive, while in half-duplex we do not. The former is not realistic. However, 
%since for larger node numbers the two modes approach each other, it can be very interesting to study distributed control in toy examples with reduced complexity, e.g. only 4 nodes with 2 slots which ``behave'' like the case for large node numbers $n$ and $\lfloor{n/2}\rfloor$ slots. \comment{OK, das ist fraglich}



%The general direction of research aimed by this work is to quantify the influence of correlations due to media access control schemes on distributed average consensus in a wireless scenario. 









%A second aspect arises when acutally verifying the theorerial findings by simulations of the consensus scenarios.  As we have briefly observed in \cite{ACC18}, rare events of ``bad behavior'' may have large impact on $r_2$ since it is a mean square measure. 
%In general, the $L^p$-joint spectral radius (in short $r_p$), $p\ge 1$, characterizes exponential stabiltiy in terms of the mean of the disagreement raised to the $p$-th power ($p$-th mean stability) \addRef{Ogura14}.
%Thus, it would of course be ideal to additionally consider $r_1$ \addRef{}, since it assigns a smaller weight to badly behaving rare events. However, $r_p$ can be computed easily only if $p$ is either even or the random measures representing the communication satisfy a certain geometric property on convex cones \addRef{Protasov} which is not the case for $r_1$ since it would then simply coincide with the essential spectral radius \addRef{Ogura14 oder LA}.

%Moreover, a computation of $r_1$ cannot constitute a full solution since the impact of rare events is already present for first mean stability, which is considered in \cite{Moura13}. There, these events are worst case paths with sub-exponential decay in disagreement and are called \textit{large deviations} stemming from the Large Deviation Theory, e.g.\addRef. The authors found that sub-exponential paths do not exist if the communication graph is connected at all instances. The latter is, however, not the case in our modelling scenario. Thus, empirical measurements of the squared disagreement cannot solely be trusted as they can suggest faster convergence than there actually is - a fact that we observe in our simulations for mean square convergence. \comment{Vergleich Bernoulli Simulation, was ist besser?}

%The question comes up why this is the case. To investigate 
%To investigate why this is the case 
%\begin{itemize}
%	\item 2-fold: Im statischen Fall tritt es schon auf \dots
%\end{itemize}

%It sheds some light on the fact
%\begin{itemize}
%	\item ICCCN-Paper stellt $k$-Schritt-Abschätzungen bereit.
%\end{itemize}
 %and investigate 
%\textbf{Outline}

\section{Related work}

The main impact on correlated packet success or - expressed in negative terms - outage correlation - in our work is due to the random set of active nodes within a slot. This kind of correlation is investigated in terms of interference in \cite{Haenggi14}
in point process settings, not for concrete deployments.
Further, it is 

In \cite{Haenggi14} intereference correlation is classified into three different types for each of which further references are provided: 1) Correlation between different time slots of a frame. We consider this type of correlation implicitly since we consider correlation of packet success between different links for the frame as a whole. 2) Correlation between different receive antennas. We consider only one antenna. 3) Correlation between different receivers: This is related to the strong component we observe between links of a common sender and different receivers.

Spatial correlation is mentioned in \addRef{}. We also observe it along the strong component.

In \cite{Ganti2009} spatial and temporal correlation of the interference in ALOHA Ad Hoc Networks is analyzed with point process methods. In contrast, we provide expressions for 
the correlation of the packet success between different links of a fixed deployment.

Correlation in communication channels can have a positive effect in communication systems. In particular for acklowledgements in broadcast communication, (little) empirical study \cite{Alam2012} (two flooding protocols are considered, one with network coding only, one with both, network coding and exploited link correlation).
Correlation of fading in MIMO systems can improve channel capacity \cite{Benef04}. In this work we broadcast study channels without acklowledgements and fading correlation. Communication channels are typically located such that they are not spatially correlated. In such systems correlation is however still present in form interference correlation due to media access. This was for example recently studied in \cite{Haenggi14} where analytical expressions on local delay and jitter \comment{weiter\dots}.
Our analytical derivations significantly differ from that work. Here we are specifically interested in the impact of interference correlation on convergence speed of average consensus using broadcast communication.

The work \cite{Kim2019} is also set in a point process setting. The authors investigate correlation to improve prediction of the packet delivery probabiltiy (PDP). Instead of computing the correlations exactly the authors approximate the correlations.

Recently, outage correlation has been investigaged in a finite point process setting (Binomial, Poisson and Thomas processes) under Rayleigh Fading \cite{Talarico2018}. Although the authors allow for (slotted) ALOHA with call occurance probability, they are mainly concerend with the spatial correlation and the effects of the spatial differences generated by the three point processes; concrete node deployments are not considered.

In\cite{Chan10}, consensus has been considered under fast fading where correlated outages (mainly due to fading) are mentioned without being quantified. In \cite{Kar2009}, \cite{Silva11} abstract correlations can be handled in the consensus framework, however neither a physical model nor a media access model is provided. Also the mean square disagreement measures used there are upper bounds only. In our work we use a different upper bound, $w_2$, \cite{ICCCN19} very well matching the shape of the exact asymptotic bound $r_2$. Both bounds together quite precisely render the outage correlation in terms of (discrete) control gain, fading parameter and number of slots utilized.
An early work meantioning the exactness of $r_2$ but rather analyzing an upper bound for the sake of simplicity is \cite{Boyd2006}.




==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/alt/30_theory.tex <==
\newpage
\ 
\newpage
\section{Background}
\subsection{Notation}
$\one$: all ones

$\ind$: indicator

$\delta_{ij}:$ Kronecker delta

Matrices $A,L$

Norms $\n{x}$, $\n{A}$


\section{Theory}
\comment{Lengthy elementary proofs will go to the appendix}
\subsection{Network model}

We assume $n$ nodes $u_1, \dots, u_n$ with fixed positions. Transmission between two nodes $u_i$ and $u_j$ is subject to path loss with a path loss coefficient of $2$. In the far field for a transmission distance $d$ the average received power is thus proportional to $1/d^2$. Let $p_{ij}$ be the average power of a transmission from $u_i$ received at $u_j$. Here we study communication under the effect of narrow band fast fading. This means that the instantaneous received power $P_{ij}$ of a transmission between $u_i$ and $u_j$ is a non-negative random variable with expectation $p_{ij}$. We employ the Nakagami fading model, i.e., the pdf $f_{ij}(x)$ of the random variable $P_{ij}$ is
\[
%f_{ij}(x) = \frac {2m^{m}}{\Gamma (m)\Omega ^{m}} x^{2m-1}\exp \left(-{\frac {m}{\Omega }}x^{2}\right)
f_{ij}(x) = \text{ind}(x>0) \frac {m^{m}\mu_{ij} ^{m}}{\Gamma (m)} x^{m-1}\exp \left(-m\mu_{ij} x\right)
\]
with shape $m \geq 1/2$ and 
    $$\mu_{ij}:= \frac{1}{P_{\text{TX}}}(4 \pi \norm{x_i - x_j}/\lambda)^2,$$
where $x_i \in\R^m$ denotes the position of node $u_i,\; \text{ind}(\cdot)$ is the indicator function, $i = 1,\dots n, $\lambda$ is the freqency
of the carrier wave and $P_{\text{TX}}$ is the transmission power which we set to a common for all nodes.

The success rate of a message transmission is modeled with outage probability under the signal plus interference to noise ratio (SINR) model. For a transmission from $u_i$ to $u_k$ all other currently ongoing transmissions will be considered as noise. Thus, we relate the received power over noise plus all other interfering transmissions as
\[
\mathrm{SINR}_{ik} = \frac{P_{ik}}{\eta + \sum_{j \in V \setminus \{ i \}} P_{jk}}
\]
where $\eta$ is a constant thermal noise term and $V$ the set of node indices of all currently transmitting nodes. We say the transmission has an outage if $\mathrm{SINR}_{ik}$ falls below a system specific threshold value $\theta > 0$. The probability of a successful packet transmission from $u_i$ to $u_k$ is
\[
\mathrm{P}[\mathrm{SINR_{ik}} \geq \theta]
\]

For media access in one round of the consensus protocol time is divided into $m$ slots. Each node chooses one of the $m$ slots uniformly distributed (i.e.\ with probability $1/m$) and independent of the other nodes' choices.

%\comment{Copied from ICCCN paper for exemplary purposes, has to be adapted!!! Continue 
%reading in the next subsection} 
%\color{blue}
%\label{subsection:SINR}
%We consider received power in a potential collision domain of $n$ nodes $u_1, \dots, u_n$ with a path loss coefficient $2.$ We consider that received power in the far field is proportional to transmit power scaled by a factor $\frac{1}{d^2}.$ One example is Friis equation with antenna gain factor $1$, i.e. received power $P_{{RX}}$ (in the far field) given by $P_{{RX}} = P_{{TX}}\cdot (\lambda/(4 \pi d))^2$ where $P_{{{TX}}}$ is the common transmit power, $d$ the sender receiver separation and $\lambda$ the carrier wave length.
%
%Let $P_{{RX}}^{ij}$ be the power received by $u_j$ of a transmission from $u_i$. We express interference from all other ongoing transmissions by the SINR model:
	%$$\text{SINR} = \frac{P_{RX}^{ik}}{N + \sum_{u_j \in V \setminus \{ u_i \}} P_{RX}^{jk}},$$
%	$$\text{SINR} = \frac{P_{RX}^{ik}}{N + \sum_{u_j \in V \setminus \{ u_i \}} P_{RX}^{jk}},$$
%where $N$ is a constant thermal noise term and $V$ is the set of all nodes transmitting at the moment. Thermal noise is given by $N = B T k_B$ where $B$ is the utilized bandwidth in Hz, $T$ the temperature in Kelvin and $k_B$ the Boltzmann constant.
%
%Packet error is modeled according to outage probability, i.e. for correct packet reception SINR has to be greater or equal a system constant $\theta$. We set $\theta$ according to Shannon capacity formula $C=B \log_2 (1+\text{SNR})$. We approximate interference as noise. Thus, given bandwidth $B$, utilized bit rate $C$ and considering $I+N$ as noise yields $\theta = 2^{C/B} - 1$. \begin{newcont} A fading margin can also be added. This, however, does not change anything for our mathematical derivation and is left out to keep the derivation uncluttered. \end{newcont}
%
%Let $m$ be a number of so called \df{slots} available in each round of the consensus protocol, and first let $m \in \N$. Slotted ALOHA means here, that at each step of the consensus iteration, all nodes independently choose one of $m$ disjoint collision domains with probability $\frac{1}{m}.$ 

Now, we discuss the transmission from node $u_i$ to $u_j,\, i\ne j.$
%Under Rayleigh fading, the probability density function (pdf) $f(x)$ of the received power $P_{RX}^{ij}$ is given by $f(x) = \mu_{ij} e^{-\mu_{ij} x} \cdot \ind$, \mbox{ where } $\ind = \left\{\begin{aligned} &1, &\mbox{ if } x > 0 \\ &0, &\mbox{ else, }   \end{aligned}$

\color{black}

\begin{prp}[\cite{ICCCN19}]
\label{prp:ICCCNprobabilites}
The probability for successful transmission from node $u_i$ to node $u_j,$ while all nodes are constantly competing for slots, is given by the formula
%$$\begin{aligned}p_{ij}(k) &= (1-\frac{1}{k}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{k (\theta + \mu_{mj} / \mu_{ij}})\right)\\
%	&=\frac{k-1}{k^{n-1}} \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(k- \frac{\theta}{\theta + \mu_{mj} / \mu_{ij}}\right)\\ &=: \sum_{m=0}^{n-1}a_{ijm}k^{-m} \end{aligned}$$
%\begin{equation}\label{eqn:p_ij}p_{ij}(m) &= (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{m (\theta + \mu_{mj} / \mu_{ij})}}\right).\end{equation}
\begin{equation}\label{eqn:p_ij}p_{ij}(m) = (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{k\ne i,j} \left(1- \frac{\theta}{m (\theta + \mu_{kj} / \mu_{ij})}\right).\end{equation}
\end{prp}


\textbf{ change: } 
Finally, we can build a Laplacian $L(m) = (\ell_{ij}(m))$ from $p_{ij}(m)$ by letting $\ell_{ij}(m) = -p_{ji}(m), i \ne j,$ and imposing the condition $L(m) \ones = 0.$

\subsection{The slot model}
\comment{
\begin{td}
	\ \\
	\begin{itemize}
		\item Mention that this is a static scenario, link to $\mu_{ij}.$
		\item Use Prop. \ref{prp:ICCCNprobabilites} as illustrative start/motivation
		%\item simplify notation: change $c_\nu := \delta_{\nu b_i}$ to $c_\nu := 1-\delta_{\nu b_i},$ thus
			%$$1-c_\nu \leadsto c_\nu$$
		\item The notation of the sum in the remark is obsolete.
		\item !!! Der Fall $m=1$ muss korrekt enthalten sein!!!
		\item Der ``Fehler'' (jetzt im Anhang) stellte das $\delta_{il}$ ein wenig in Frage. Nochmal den Fehler nachvollziehen und gucken, was im Fall $i=l$ ist.
	\end{itemize}
\end{td}}
Let $u_1, \dots, u_n$ be $n\ge 2$ nodes, let $m \in \N$ be the number of available contention windows (in the following simply called \textit{slots}), denote by $N$ the thermal noise and denote by $\theta \in \R_+$ the SINR threshold. We require $\theta \ge 1$ and $N>0$ Watt. Let us further introduce $n$ independent random variables $S_1,\dots, S_n$ representing each node's choice of slot - all equally likely - i.e. $S_i \sim unif(\{1, \dots, m\}), \; i = 1 ,\dots n.$

Denote by $P_{ij}, \, 1 \le i, j \le n,\; i \ne j,$ the power received at node $u_j$ if some different node $u_i$ is solely transmitting, subject to path loss and fading (the notation shall not be affected if there are actually other nodes sending in which case $P_{ij}$ is just the received power fraction due to node $u_i$). In this work we will consider Gamma distributed (Nakagami fading) and (non-central) chi-square distributed (Ricean fading) powers. However, theoretical considerations are limited to Nakagami fading to keep mathematics tractable, although the slot model yields general expressions independent of the fading distribution (see Prop. \ref{prp:slotCorrelations}). 

Moreover we assume the power variables to be independent (\comment{Add justification, ref to ICCCN-Paper? \cite{ICCCN19}}). We can now express power and interference in slot $k, \; 1 \le k \le m:$
	$$P_{ij}^{k} := \delta_{S_i k} P_{ij} \ds \mbox{ and }\ds I_{ij}^k := \sum_{\substack{l=1 \\ l\ne i,j}}^{n}P_{lj}^{k}.$$
Let us introduce random variables for excess of the SINR threshold in slot $k$ and in any slot respectively:
	$$X_{ij}^k := \ind\left(\frac{P_{ij}^k}{N + I_{ij}^k}\ge \theta  \right) \ds \mbox{ and } \ds X_{ij} := \sum_{k=1}^{m} X_{ij}^k.$$
	Clearly, from the definition of $P_{ij}^k$ and the fact that $\theta, (N + I_{ij}^k) >0$ we have $X_{ij}^k = \delta_{S_i k} \cdot X_{ij}^k,$ thus $X_{ij} = X_{ij}^{S_i}.$

There are two further aspects we have to consider: Sending nodes cannot receive (singular antenna case) and multiple receptions at some node at the same time (i.e. in the same slot) are impossible (\comment{improvement?}). We will only model the former aspect in our formal treatment. However, we keep track of the latter case in simulations and show (\comment{verify!!}) that this happens rarely such that our analysis is still meaningful. \comment{Maybe also add estimates somewhere}. In this sense we define successful packet reception $Y_{ij}, \, 1 \le i, j \le n,\; i \ne j,$ as Bernoulli variable having the property to vanish if $u_i$ and $u_j$ chose the same slot:
    $$ Y_{ij} := (1-\delta_{S_i S_j}) \cdot X_{ij} \ds\ds 1 \le i,j \le n, i\ne j.$$
    

The mixed moments of the $X_{ij}$'s are of special importance to calculate the covariance. 
By the law of total probability we can decompose $\E X_{ij}X_{kl},\, i \ne k,$ as
$$ \frac{1}{m} \cdot \E[X_{ij}X_{kl}\vert S_{i} = S_{k}] + (1-\frac{1}{m})\E[X_{ij}X_{kl}\vert S_{i} \ne S_{k}]$$
which motivates the next Proposition whose proof is defered until the Appendix.
\begin{prp}

\label{prp:slotCorrelations}
Let $\theta \ge 1,$ let $N > 0$, let $i \ne j, k \ne l,$ and $(i,j) \ne (k,l),$ and define
\begin{equation}\begin{aligned}\label{eqn:formulaSameSlot}\Phi_{ijkl}  :=  \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijk}(c)\cdot \alpha_{kli}(c) \end{aligned}\end{equation}
and
	$$\Psi_{ijkl} :=\prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c),$$ 
where\footnote{the product with subsequent sum (e.g. in (\ref{eqn:formulaSameSlot})) is meant to expand into an $n-2$-fold sum over $c_\nu,\ \nu \ne i,k.$}
\begin{subequations}\begin{align}\label{eqn:alpha_phi} \phi(c) &:= \prod_{\nu \ne i,k}(m-1)^{1-c_\nu},\\
		\psi(c) &:= \prod_{\substack{\nu = 1\\ \nu \ne i,k}}^n (m-2)^{\delta_{c_\nu, 0}}\\
			%\alpha_{i'j'}(c) &: = \Pr\left(\frac{P_{i'j'}}{N+\sum_{\nu\ne i',j'}^{}c_\nu P_{\nu j'}} \ge \theta\right),\\
			%\alpha_{xy}(c) &: = \Pr\left(\frac{P_{xy}}{N+\sum_{\nu\ne x,y}^{}c_\nu P_{\nu y}} \ge \theta\right),
		\alpha_{xyz}(c) &= \Pr\left(\frac{P_{xy}}{N+\sum\limits_{\nu\ne x,y,z}^{}c_\nu P_{\nu y} + (1-\delta_{xz})P_{zy}} \ge \theta\right)\\
	\beta_{i'j'k'}^{(d)}(c) &: = \Pr\left(\frac{P_{i'j'}}{N+\sum_{\nu\ne i',j',k'}^{}\delta_{c_\nu d} P_{\nu j'}} \ge \theta  \right),\\
\end{align}\end{subequations}
$d = 1,2$ and where $c = (c_\nu) \in   \left\{ 0,1 \right\}^{n-2+\delta_{ik}},$
	$$c = (c_1, \dots, c_{\mu-1},c_{\mu+1},\dots, c_{M-1}, c_{M+1},\dots, c_n),$$
$\mu = \mbox{min}(i,k), M = \mbox{max}(i,k).$   

\begin{abc}\item Then we have 
		$$\E[X_{ij}X_{kl} \vert S_i = S_k] = \frac{1-\delta_{lj}}{m^{n-2+\delta_{ik}}} \cdot \Phi_{ijkl}.$$
		In particular, $\E X_{ij}X_{il} = \E [X_{ij}X_{il} \vert S_i = S_i]$ can be expressed in virtue of (\ref{eqn:formulaSameSlot}) which gives for $j \ne l$
		$$\cov(X_{ij}, X_{il}) = \frac{ \Phi_{ijil}}{m^{n-2+\delta_{ik}}}  - \E X_{ij} \E X_{kl}.$$


  	%\item For $k\ne i, l \ne j, i\ne l, k\ne j$ we have
  	\item For $k\ne i,$
		%$$ \begin{aligned}&\E [X_{ij}X_{kl}\vert S_i \ne S_k]  = \frac{1}{(m-1)m^{n-1}}\cdot \Psi_{ijkl}
		$$ \begin{aligned}&\E [X_{ij}X_{kl}\vert S_i \ne S_k]  = \frac{1}{m^{n-2}}\cdot \Psi_{ijkl}
			%&= \frac{1}{(m-1)m^{n-1}} \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
			,\end{aligned}$$
		hence
		    $$\begin{aligned} \cov(X_{ij}, X_{kl}) &= \frac{1-\delta_{lj}}{m^{n}} \cdot \Phi_{ijkl}+ \frac{m-1}{ m^{n-1}}\cdot \Psi_{ijkl} \\
		    &\;\,\;  - \E X_{ij} \E X_{kl}.  \end{aligned}$$
	\end{abc}
\end{prp}
%\begin{proof}
%See Appendix.	
%\end{proof} 




\begin{rem}
	\begin{abc}
	\item The requirement $\theta \ge 1$ is used only in the case $l = j$ and yields the $(1-\delta_{lj})$ factor/minuend.
	\item In case $m=1$ we have $\Phi_{ijkl} = \E X_{ij} \E X_{kl}$ \comment{(verify!)} and so ``everything is independent as expected'' \comment{(verify!!)}
 	\item Since the summations can get large it is important to efficiently implement the sums. E.g. $\csum{1}\left( \dots \right)$ can be implemented using a loop from 1 to $2^{n-2}$ over a variable $i$ and accessing the ``components'' $c_{\iota}$ of $i$ by bitwise operations (bit-shift).
 
	\end{abc}
\end{rem} 

\begin{proof}[Proof of Proposition \ref{prp:slotCorrelations}]
\begin{abc}
	\item Let $i \ne j, k\ne l.$ Assume first $i \ne k.$ Then
		$$\begin{aligned} &\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right] \\
			&= \Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j}}^{n}\delta_{S_i S_\nu} \cdot P_{\nu j}} \ge \theta \mbox{ and } \right.\\
			&\left.\left. \ds \ds \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l}}^{n}\delta_{S_k S_\nu} \cdot P_{\nu l}} \ge \theta  \right\vert S_i = S_k \right)\\
			&= \frac{1}{m^{n-1}} \sum_{\substack{b_i = 1\\ (b_i = b_k)}}^{m}\sum_{\substack{b_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu j} + P_{kj}} \ge \theta \mbox{ and } \right.\\ 
			&\left. \ds \ds \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu l} + P_{il}} \ge \theta  \right)\\
		\end{aligned}$$
	In case $j = l,$ observe that we have the following situation, with $a,b > 0$ appropriately set:
		$$\Pr\left( \frac{a}{N+b} \ge \theta \mbox{ and }  \frac{b}{N + a} \ge \theta  \right) = 0,$$
	since $\frac{a}{N+b} \ge \theta \mbox{ and }  \frac{b}{N + a} \ge \theta$ implies 
		$$ a \ge \theta (N + \theta(N+a)) = \theta N + \theta^2 N + \theta^2a.$$
	which leads to the contradiction
		$$(1-\theta^2) a \ge \theta N (1+\theta)$$
		since $\theta \ge 1.$ Hence we have to add the prefactor $1- \delta_{jl}:$
		$$\begin{aligned} &\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right] \\
			&= \frac{1- \delta_{jl}}{m^{n-1}} \sum_{\substack{b_i = 1\\ (b_i = b_k)}}^{m}\sum_{\substack{b_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu j} + P_{kj}} \ge \theta \right)\\ 
			& \ds \ds \cdot \Pr\left(\frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu l} + P_{il}} \ge \theta  \right),\\
		\end{aligned}$$ 
		where we have already exploited the independence \comment{(describe in more detail)} in case $j \ne l$ splitting the summands into two probability factors. Inspection of the summands reveals that the $m^{n-1}$ states of the $b_\nu$'s$, \nu \ne k$ can be cast into $n-2$ macro state variables $c_\nu = 0, 1,\; \nu \in \left\{ 1, \dots, n  \right\}\setminus \{i,k\} $ representing the cases $b_i \ne b_\nu$ and $b_i = b_\nu$ respectively. For each $b_\nu$ the former case has $n-1$ realizations while for the latter there is only one. Thus, the combined weight for the macro state $c = (c_{\nu}), \nu \ne i,k,$ is 
		$$\phi(c) = \prod_{\nu \ne i,k}(m-1)^{1-c_\nu}.$$
We can now express $\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right]$ in terms of the macro states:
$$ \begin{aligned}&\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right] \\
	& = \frac{1- \delta_{jl}}{m^{n-1}} \sum_{\substack{b_i = 1\\ (b_i = b_k)}}^{m}\sum_{\substack{c_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}c_{\nu} \cdot P_{\nu j} + P_{kj}} \ge \theta \right)\\ 
	&\ds \ds \cdot \Pr\left(\frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}c_{\nu} \cdot P_{\nu l} + P_{il}} \ge \theta  \right),\\
 	& =  \frac{1- \delta_{jl}}{m^{n-1}} \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijk}(c)\cdot \alpha_{kli}(c) \end{aligned},$$
where the case $i = k$ is already incorporated using the Kronecker deltas of the $\alpha_{i'j'k'}$'s \comment{(improve)}.
 
	\item Let $i \ne k.$ Then
		$$\begin{aligned}&\E\left[ X_{ij}X_{kl}\vert S_i \ne S_k \right]\\
			&= \Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j}}^{n}\delta_{S_i S_\nu} \cdot P_{\nu j}} \ge \theta \mbox{ and } \right.\\
			&\left.\left. \ds \ds \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l}}^{n}\delta_{S_k S_\nu} \cdot P_{\nu l}} \ge \theta  \right\vert S_i \ne S_k \right)\\
		&= \frac{1}{m^{n-1}(m-1)} \sum_{\substack{b_i, b_k = 1\\ b_i \ne b_k}}^{m}\sum_{\substack{b_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu j}} \ge \theta \right)\\
			&\ds \ds \cdot \Pr\left( \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{b_k b_\nu} \cdot P_{\nu l}} \ge \theta  \right)\\
			&= \frac{1}{m^{n-1}(m-1)} \sum_{\substack{b_i, b_k = 1\\ b_i \ne b_k}}^{m}\sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^{2}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{c_\nu 1} \cdot P_{\nu j}} \ge \theta \right) \\
			&\ds \ds \cdot \Pr\left( \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{c_\nu 2} \cdot P_{\nu l}} \ge \theta  \right)\cdot \psi(c)\\
			&= \frac{1}{m^{n-1}(m-1)} \sum_{\substack{b_i, b_k = 1\\ b_i \ne b_k}}^{m}\sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^{2} \psi(c) \cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
			&= \frac{1}{m^{n-2}} \sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^{2} \psi(c) \cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
		\end{aligned},$$ 
\end{abc}
where we have introduced the macro states $c_{\nu}.$ The state $c_\nu = 1$ represents the case $b_\nu = b_i$, the state $c_\nu = 2$ represents the case $b_\nu = b_k,$ and the state $c_\nu = 0$ representes any other case. Hence the weights for $c_\nu = 0, 1, 2$ are $m-2, 1, 1$ respectively which are gathered in the factor $\psi(c).$

\end{proof} 



\begin{cor}[Nakagami-m Fading, \cite{Nakagami12}]
	$$\E X_{ij} = \cdots $$
and
    $$\alpha_{i'j'k'}= \cdots$$
    $$\beta_{i'j'k'}= \cdots$$
	
	
	\comment{Currently, only the part where sending and receiving is allowed (so the prefactor of the ICCCN formula is missing in this result)}
\end{cor}

\begin{rem}
For Nakagami-Parameter=1 (Rayleigh fading) we recover the probabilities of [ICCCN19] for the full duplex case, i.e. ignoring the prefactor.   
\end{rem}
\begin{proof}
	$$\begin{aligned} \E X_{ij} = \E X_{ij}^{S_i} &= P(\frac{P_{ij}}{N+\sum_{l\ne i,j}\delta_{S_l S_i} P_{l j}} \ge \theta)\\
		&= \E \prod_{l\ne i,j}\exp\left\{ -\mu_{i j} \theta(N+ \delta_{S_i S_l} P_{l j})  \right\}\\
		&= \prod_{l\ne i,j} \E \exp\left\{ -\mu_{i j} \theta(N+ \delta_{S_i S_l} P_{l j})  \right\}\\
		&= \frac{1}{m^2} e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \sum_{\nu,\mu = 1}^{m}\E \exp\left\{ -\mu_{\nu j } \theta \delta_{\nu \mu} P_{l j} \right\}\\
		&= \frac{1}{m^2} e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( (m^2 - m) + \sum_{\nu=1}^{m} \E e^{-\mu_{i j}\theta P_{lj}} \right)\\
		&=  e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( (1-\frac{1}{m}) + \frac{1}{m}\cdot\frac{1}{1+\theta \frac{\mu_{i j}}{\mu_{lj}}} \right)\\
		&=  e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( 1 - \frac{1}{m}\cdot \frac{\theta \frac{\mu_{i j}}{\mu_{lj}}}{\theta \frac{\mu_{i j}}{\mu_{lj}} +1} \right)\\
		&=  e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( 1 - \frac{1}{m} \cdot \frac{\theta}{\theta + \frac{\mu_{lj}}{ \mu_{i j} }} \right)
	\end{aligned}$$
 \end{proof}




==> Outage%20Correlation%20inRandom%20Media%20Access%20with%20Application%20to%20AverageConsensus%20(CamReady)/copyright.tex <==
 \twocolumn[
  \begin{@twocolumnfalse}
 
 
 \large
This  paper  is  a  preprint  (IEEE  “accepted”  status). IEEE copyright notice. \copyright 2015
IEEE. Personal use of this material is permitted. Permission from IEEE must be
obtained for all other uses, in any current or future media, including
reprinting/republishing this material for advertising or promotional purposes,
creating new collective works, for resale or redistribution to servers or lists, or
reuse of any copyrighted.
 \end{@twocolumnfalse}
]
\newpage

==> alt/30_theory.tex <==
\newpage
\ 
\newpage
\section{Background}
\subsection{Notation}
$\one$: all ones

$\ind$: indicator

$\delta_{ij}:$ Kronecker delta

Matrices $A,L$

Norms $\n{x}$, $\n{A}$


\section{Theory}
\comment{Lengthy elementary proofs will go to the appendix}
\subsection{Network model}

We assume $n$ nodes $u_1, \dots, u_n$ with fixed positions. Transmission between two nodes $u_i$ and $u_j$ is subject to path loss with a path loss coefficient of $2$. In the far field for a transmission distance $d$ the average received power is thus proportional to $1/d^2$. Let $p_{ij}$ be the average power of a transmission from $u_i$ received at $u_j$. Here we study communication under the effect of narrow band fast fading. This means that the instantaneous received power $P_{ij}$ of a transmission between $u_i$ and $u_j$ is a non-negative random variable with expectation $p_{ij}$. We employ the Nakagami fading model, i.e., the pdf $f_{ij}(x)$ of the random variable $P_{ij}$ is
\[
%f_{ij}(x) = \frac {2m^{m}}{\Gamma (m)\Omega ^{m}} x^{2m-1}\exp \left(-{\frac {m}{\Omega }}x^{2}\right)
f_{ij}(x) = \text{ind}(x>0) \frac {m^{m}\mu_{ij} ^{m}}{\Gamma (m)} x^{m-1}\exp \left(-m\mu_{ij} x\right)
\]
with shape $m \geq 1/2$ and 
    $$\mu_{ij}:= \frac{1}{P_{\text{TX}}}(4 \pi \norm{x_i - x_j}/\lambda)^2,$$
where $x_i \in\R^m$ denotes the position of node $u_i,\; \text{ind}(\cdot)$ is the indicator function, $i = 1,\dots n, $\lambda$ is the freqency
of the carrier wave and $P_{\text{TX}}$ is the transmission power which we set to a common for all nodes.

The success rate of a message transmission is modeled with outage probability under the signal plus interference to noise ratio (SINR) model. For a transmission from $u_i$ to $u_k$ all other currently ongoing transmissions will be considered as noise. Thus, we relate the received power over noise plus all other interfering transmissions as
\[
\mathrm{SINR}_{ik} = \frac{P_{ik}}{\eta + \sum_{j \in V \setminus \{ i \}} P_{jk}}
\]
where $\eta$ is a constant thermal noise term and $V$ the set of node indices of all currently transmitting nodes. We say the transmission has an outage if $\mathrm{SINR}_{ik}$ falls below a system specific threshold value $\theta > 0$. The probability of a successful packet transmission from $u_i$ to $u_k$ is
\[
\mathrm{P}[\mathrm{SINR_{ik}} \geq \theta]
\]

For media access in one round of the consensus protocol time is divided into $m$ slots. Each node chooses one of the $m$ slots uniformly distributed (i.e.\ with probability $1/m$) and independent of the other nodes' choices.

%\comment{Copied from ICCCN paper for exemplary purposes, has to be adapted!!! Continue 
%reading in the next subsection} 
%\color{blue}
%\label{subsection:SINR}
%We consider received power in a potential collision domain of $n$ nodes $u_1, \dots, u_n$ with a path loss coefficient $2.$ We consider that received power in the far field is proportional to transmit power scaled by a factor $\frac{1}{d^2}.$ One example is Friis equation with antenna gain factor $1$, i.e. received power $P_{{RX}}$ (in the far field) given by $P_{{RX}} = P_{{TX}}\cdot (\lambda/(4 \pi d))^2$ where $P_{{{TX}}}$ is the common transmit power, $d$ the sender receiver separation and $\lambda$ the carrier wave length.
%
%Let $P_{{RX}}^{ij}$ be the power received by $u_j$ of a transmission from $u_i$. We express interference from all other ongoing transmissions by the SINR model:
	%$$\text{SINR} = \frac{P_{RX}^{ik}}{N + \sum_{u_j \in V \setminus \{ u_i \}} P_{RX}^{jk}},$$
%	$$\text{SINR} = \frac{P_{RX}^{ik}}{N + \sum_{u_j \in V \setminus \{ u_i \}} P_{RX}^{jk}},$$
%where $N$ is a constant thermal noise term and $V$ is the set of all nodes transmitting at the moment. Thermal noise is given by $N = B T k_B$ where $B$ is the utilized bandwidth in Hz, $T$ the temperature in Kelvin and $k_B$ the Boltzmann constant.
%
%Packet error is modeled according to outage probability, i.e. for correct packet reception SINR has to be greater or equal a system constant $\theta$. We set $\theta$ according to Shannon capacity formula $C=B \log_2 (1+\text{SNR})$. We approximate interference as noise. Thus, given bandwidth $B$, utilized bit rate $C$ and considering $I+N$ as noise yields $\theta = 2^{C/B} - 1$. \begin{newcont} A fading margin can also be added. This, however, does not change anything for our mathematical derivation and is left out to keep the derivation uncluttered. \end{newcont}
%
%Let $m$ be a number of so called \df{slots} available in each round of the consensus protocol, and first let $m \in \N$. Slotted ALOHA means here, that at each step of the consensus iteration, all nodes independently choose one of $m$ disjoint collision domains with probability $\frac{1}{m}.$ 

Now, we discuss the transmission from node $u_i$ to $u_j,\, i\ne j.$
%Under Rayleigh fading, the probability density function (pdf) $f(x)$ of the received power $P_{RX}^{ij}$ is given by $f(x) = \mu_{ij} e^{-\mu_{ij} x} \cdot \ind$, \mbox{ where } $\ind = \left\{\begin{aligned} &1, &\mbox{ if } x > 0 \\ &0, &\mbox{ else, }   \end{aligned}$

\color{black}

\begin{prp}[\cite{ICCCN19}]
\label{prp:ICCCNprobabilites}
The probability for successful transmission from node $u_i$ to node $u_j,$ while all nodes are constantly competing for slots, is given by the formula
%$$\begin{aligned}p_{ij}(k) &= (1-\frac{1}{k}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{k (\theta + \mu_{mj} / \mu_{ij}})\right)\\
%	&=\frac{k-1}{k^{n-1}} \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(k- \frac{\theta}{\theta + \mu_{mj} / \mu_{ij}}\right)\\ &=: \sum_{m=0}^{n-1}a_{ijm}k^{-m} \end{aligned}$$
%\begin{equation}\label{eqn:p_ij}p_{ij}(m) &= (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{\scriptsize\begin{aligned}m=1\\ m\ne i,j\end{aligned}}^n \left(1- \frac{\theta}{m (\theta + \mu_{mj} / \mu_{ij})}}\right).\end{equation}
\begin{equation}\label{eqn:p_ij}p_{ij}(m) = (1-\frac{1}{m}) \cdot e^{ -\mu_{ij} \theta \cdot N } \prod_{k\ne i,j} \left(1- \frac{\theta}{m (\theta + \mu_{kj} / \mu_{ij})}\right).\end{equation}
\end{prp}


\textbf{ change: } 
Finally, we can build a Laplacian $L(m) = (\ell_{ij}(m))$ from $p_{ij}(m)$ by letting $\ell_{ij}(m) = -p_{ji}(m), i \ne j,$ and imposing the condition $L(m) \ones = 0.$

\subsection{The slot model}
\comment{
\begin{td}
	\ \\
	\begin{itemize}
		\item Mention that this is a static scenario, link to $\mu_{ij}.$
		\item Use Prop. \ref{prp:ICCCNprobabilites} as illustrative start/motivation
		%\item simplify notation: change $c_\nu := \delta_{\nu b_i}$ to $c_\nu := 1-\delta_{\nu b_i},$ thus
			%$$1-c_\nu \leadsto c_\nu$$
		\item The notation of the sum in the remark is obsolete.
		\item !!! Der Fall $m=1$ muss korrekt enthalten sein!!!
		\item Der ``Fehler'' (jetzt im Anhang) stellte das $\delta_{il}$ ein wenig in Frage. Nochmal den Fehler nachvollziehen und gucken, was im Fall $i=l$ ist.
	\end{itemize}
\end{td}}
Let $u_1, \dots, u_n$ be $n\ge 2$ nodes, let $m \in \N$ be the number of available contention windows (in the following simply called \textit{slots}), denote by $N$ the thermal noise and denote by $\theta \in \R_+$ the SINR threshold. We require $\theta \ge 1$ and $N>0$ Watt. Let us further introduce $n$ independent random variables $S_1,\dots, S_n$ representing each node's choice of slot - all equally likely - i.e. $S_i \sim unif(\{1, \dots, m\}), \; i = 1 ,\dots n.$

Denote by $P_{ij}, \, 1 \le i, j \le n,\; i \ne j,$ the power received at node $u_j$ if some different node $u_i$ is solely transmitting, subject to path loss and fading (the notation shall not be affected if there are actually other nodes sending in which case $P_{ij}$ is just the received power fraction due to node $u_i$). In this work we will consider Gamma distributed (Nakagami fading) and (non-central) chi-square distributed (Ricean fading) powers. However, theoretical considerations are limited to Nakagami fading to keep mathematics tractable, although the slot model yields general expressions independent of the fading distribution (see Prop. \ref{prp:slotCorrelations}). 

Moreover we assume the power variables to be independent (\comment{Add justification, ref to ICCCN-Paper? \cite{ICCCN19}}). We can now express power and interference in slot $k, \; 1 \le k \le m:$
	$$P_{ij}^{k} := \delta_{S_i k} P_{ij} \ds \mbox{ and }\ds I_{ij}^k := \sum_{\substack{l=1 \\ l\ne i,j}}^{n}P_{lj}^{k}.$$
Let us introduce random variables for excess of the SINR threshold in slot $k$ and in any slot respectively:
	$$X_{ij}^k := \ind\left(\frac{P_{ij}^k}{N + I_{ij}^k}\ge \theta  \right) \ds \mbox{ and } \ds X_{ij} := \sum_{k=1}^{m} X_{ij}^k.$$
	Clearly, from the definition of $P_{ij}^k$ and the fact that $\theta, (N + I_{ij}^k) >0$ we have $X_{ij}^k = \delta_{S_i k} \cdot X_{ij}^k,$ thus $X_{ij} = X_{ij}^{S_i}.$

There are two further aspects we have to consider: Sending nodes cannot receive (singular antenna case) and multiple receptions at some node at the same time (i.e. in the same slot) are impossible (\comment{improvement?}). We will only model the former aspect in our formal treatment. However, we keep track of the latter case in simulations and show (\comment{verify!!}) that this happens rarely such that our analysis is still meaningful. \comment{Maybe also add estimates somewhere}. In this sense we define successful packet reception $Y_{ij}, \, 1 \le i, j \le n,\; i \ne j,$ as Bernoulli variable having the property to vanish if $u_i$ and $u_j$ chose the same slot:
    $$ Y_{ij} := (1-\delta_{S_i S_j}) \cdot X_{ij} \ds\ds 1 \le i,j \le n, i\ne j.$$
    

The mixed moments of the $X_{ij}$'s are of special importance to calculate the covariance. 
By the law of total probability we can decompose $\E X_{ij}X_{kl},\, i \ne k,$ as
$$ \frac{1}{m} \cdot \E[X_{ij}X_{kl}\vert S_{i} = S_{k}] + (1-\frac{1}{m})\E[X_{ij}X_{kl}\vert S_{i} \ne S_{k}]$$
which motivates the next Proposition whose proof is defered until the Appendix.
\begin{prp}

\label{prp:slotCorrelations}
Let $\theta \ge 1,$ let $N > 0$, let $i \ne j, k \ne l,$ and $(i,j) \ne (k,l),$ and define
\begin{equation}\begin{aligned}\label{eqn:formulaSameSlot}\Phi_{ijkl}  :=  \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijk}(c)\cdot \alpha_{kli}(c) \end{aligned}\end{equation}
and
	$$\Psi_{ijkl} :=\prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c),$$ 
where\footnote{the product with subsequent sum (e.g. in (\ref{eqn:formulaSameSlot})) is meant to expand into an $n-2$-fold sum over $c_\nu,\ \nu \ne i,k.$}
\begin{subequations}\begin{align}\label{eqn:alpha_phi} \phi(c) &:= \prod_{\nu \ne i,k}(m-1)^{1-c_\nu},\\
		\psi(c) &:= \prod_{\substack{\nu = 1\\ \nu \ne i,k}}^n (m-2)^{\delta_{c_\nu, 0}}\\
			%\alpha_{i'j'}(c) &: = \Pr\left(\frac{P_{i'j'}}{N+\sum_{\nu\ne i',j'}^{}c_\nu P_{\nu j'}} \ge \theta\right),\\
			%\alpha_{xy}(c) &: = \Pr\left(\frac{P_{xy}}{N+\sum_{\nu\ne x,y}^{}c_\nu P_{\nu y}} \ge \theta\right),
		\alpha_{xyz}(c) &= \Pr\left(\frac{P_{xy}}{N+\sum\limits_{\nu\ne x,y,z}^{}c_\nu P_{\nu y} + (1-\delta_{xz})P_{zy}} \ge \theta\right)\\
	\beta_{i'j'k'}^{(d)}(c) &: = \Pr\left(\frac{P_{i'j'}}{N+\sum_{\nu\ne i',j',k'}^{}\delta_{c_\nu d} P_{\nu j'}} \ge \theta  \right),\\
\end{align}\end{subequations}
$d = 1,2$ and where $c = (c_\nu) \in   \left\{ 0,1 \right\}^{n-2+\delta_{ik}},$
	$$c = (c_1, \dots, c_{\mu-1},c_{\mu+1},\dots, c_{M-1}, c_{M+1},\dots, c_n),$$
$\mu = \mbox{min}(i,k), M = \mbox{max}(i,k).$   

\begin{abc}\item Then we have 
		$$\E[X_{ij}X_{kl} \vert S_i = S_k] = \frac{1-\delta_{lj}}{m^{n-2+\delta_{ik}}} \cdot \Phi_{ijkl}.$$
		In particular, $\E X_{ij}X_{il} = \E [X_{ij}X_{il} \vert S_i = S_i]$ can be expressed in virtue of (\ref{eqn:formulaSameSlot}) which gives for $j \ne l$
		$$\cov(X_{ij}, X_{il}) = \frac{ \Phi_{ijil}}{m^{n-2+\delta_{ik}}}  - \E X_{ij} \E X_{kl}.$$


  	%\item For $k\ne i, l \ne j, i\ne l, k\ne j$ we have
  	\item For $k\ne i,$
		%$$ \begin{aligned}&\E [X_{ij}X_{kl}\vert S_i \ne S_k]  = \frac{1}{(m-1)m^{n-1}}\cdot \Psi_{ijkl}
		$$ \begin{aligned}&\E [X_{ij}X_{kl}\vert S_i \ne S_k]  = \frac{1}{m^{n-2}}\cdot \Psi_{ijkl}
			%&= \frac{1}{(m-1)m^{n-1}} \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{2}  \psi(c)\cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
			,\end{aligned}$$
		hence
		    $$\begin{aligned} \cov(X_{ij}, X_{kl}) &= \frac{1-\delta_{lj}}{m^{n}} \cdot \Phi_{ijkl}+ \frac{m-1}{ m^{n-1}}\cdot \Psi_{ijkl} \\
		    &\;\,\;  - \E X_{ij} \E X_{kl}.  \end{aligned}$$
	\end{abc}
\end{prp}
%\begin{proof}
%See Appendix.	
%\end{proof} 




\begin{rem}
	\begin{abc}
	\item The requirement $\theta \ge 1$ is used only in the case $l = j$ and yields the $(1-\delta_{lj})$ factor/minuend.
	\item In case $m=1$ we have $\Phi_{ijkl} = \E X_{ij} \E X_{kl}$ \comment{(verify!)} and so ``everything is independent as expected'' \comment{(verify!!)}
 	\item Since the summations can get large it is important to efficiently implement the sums. E.g. $\csum{1}\left( \dots \right)$ can be implemented using a loop from 1 to $2^{n-2}$ over a variable $i$ and accessing the ``components'' $c_{\iota}$ of $i$ by bitwise operations (bit-shift).
 
	\end{abc}
\end{rem} 

\begin{proof}[Proof of Proposition \ref{prp:slotCorrelations}]
\begin{abc}
	\item Let $i \ne j, k\ne l.$ Assume first $i \ne k.$ Then
		$$\begin{aligned} &\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right] \\
			&= \Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j}}^{n}\delta_{S_i S_\nu} \cdot P_{\nu j}} \ge \theta \mbox{ and } \right.\\
			&\left.\left. \ds \ds \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l}}^{n}\delta_{S_k S_\nu} \cdot P_{\nu l}} \ge \theta  \right\vert S_i = S_k \right)\\
			&= \frac{1}{m^{n-1}} \sum_{\substack{b_i = 1\\ (b_i = b_k)}}^{m}\sum_{\substack{b_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu j} + P_{kj}} \ge \theta \mbox{ and } \right.\\ 
			&\left. \ds \ds \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu l} + P_{il}} \ge \theta  \right)\\
		\end{aligned}$$
	In case $j = l,$ observe that we have the following situation, with $a,b > 0$ appropriately set:
		$$\Pr\left( \frac{a}{N+b} \ge \theta \mbox{ and }  \frac{b}{N + a} \ge \theta  \right) = 0,$$
	since $\frac{a}{N+b} \ge \theta \mbox{ and }  \frac{b}{N + a} \ge \theta$ implies 
		$$ a \ge \theta (N + \theta(N+a)) = \theta N + \theta^2 N + \theta^2a.$$
	which leads to the contradiction
		$$(1-\theta^2) a \ge \theta N (1+\theta)$$
		since $\theta \ge 1.$ Hence we have to add the prefactor $1- \delta_{jl}:$
		$$\begin{aligned} &\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right] \\
			&= \frac{1- \delta_{jl}}{m^{n-1}} \sum_{\substack{b_i = 1\\ (b_i = b_k)}}^{m}\sum_{\substack{b_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu j} + P_{kj}} \ge \theta \right)\\ 
			& \ds \ds \cdot \Pr\left(\frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu l} + P_{il}} \ge \theta  \right),\\
		\end{aligned}$$ 
		where we have already exploited the independence \comment{(describe in more detail)} in case $j \ne l$ splitting the summands into two probability factors. Inspection of the summands reveals that the $m^{n-1}$ states of the $b_\nu$'s$, \nu \ne k$ can be cast into $n-2$ macro state variables $c_\nu = 0, 1,\; \nu \in \left\{ 1, \dots, n  \right\}\setminus \{i,k\} $ representing the cases $b_i \ne b_\nu$ and $b_i = b_\nu$ respectively. For each $b_\nu$ the former case has $n-1$ realizations while for the latter there is only one. Thus, the combined weight for the macro state $c = (c_{\nu}), \nu \ne i,k,$ is 
		$$\phi(c) = \prod_{\nu \ne i,k}(m-1)^{1-c_\nu}.$$
We can now express $\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right]$ in terms of the macro states:
$$ \begin{aligned}&\E \left[ X_{ij} X_{kl} \mid S_i = S_k \right] \\
	& = \frac{1- \delta_{jl}}{m^{n-1}} \sum_{\substack{b_i = 1\\ (b_i = b_k)}}^{m}\sum_{\substack{c_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}c_{\nu} \cdot P_{\nu j} + P_{kj}} \ge \theta \right)\\ 
	&\ds \ds \cdot \Pr\left(\frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}c_{\nu} \cdot P_{\nu l} + P_{il}} \ge \theta  \right),\\
 	& =  \frac{1- \delta_{jl}}{m^{n-1}} \prod_{\substack{\nu = 1\\ \nu\ne i,k }}^n \sum_{c_\nu=0}^{1}\phi(c)\cdot \alpha_{ijk}(c)\cdot \alpha_{kli}(c) \end{aligned},$$
where the case $i = k$ is already incorporated using the Kronecker deltas of the $\alpha_{i'j'k'}$'s \comment{(improve)}.
 
	\item Let $i \ne k.$ Then
		$$\begin{aligned}&\E\left[ X_{ij}X_{kl}\vert S_i \ne S_k \right]\\
			&= \Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j}}^{n}\delta_{S_i S_\nu} \cdot P_{\nu j}} \ge \theta \mbox{ and } \right.\\
			&\left.\left. \ds \ds \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l}}^{n}\delta_{S_k S_\nu} \cdot P_{\nu l}} \ge \theta  \right\vert S_i \ne S_k \right)\\
		&= \frac{1}{m^{n-1}(m-1)} \sum_{\substack{b_i, b_k = 1\\ b_i \ne b_k}}^{m}\sum_{\substack{b_\nu = 1\\ \nu \ne i,k}}^{m}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{b_i b_\nu} \cdot P_{\nu j}} \ge \theta \right)\\
			&\ds \ds \cdot \Pr\left( \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{b_k b_\nu} \cdot P_{\nu l}} \ge \theta  \right)\\
			&= \frac{1}{m^{n-1}(m-1)} \sum_{\substack{b_i, b_k = 1\\ b_i \ne b_k}}^{m}\sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^{2}\Pr\left( \frac{P_{ij}}{N + \sum_{\substack{\nu= 1\\\nu\ne i,j,k}}^{n}\delta_{c_\nu 1} \cdot P_{\nu j}} \ge \theta \right) \\
			&\ds \ds \cdot \Pr\left( \frac{P_{kl}}{N + \sum_{\substack{\nu= 1\\\nu\ne k,l,i}}^{n}\delta_{c_\nu 2} \cdot P_{\nu l}} \ge \theta  \right)\cdot \psi(c)\\
			&= \frac{1}{m^{n-1}(m-1)} \sum_{\substack{b_i, b_k = 1\\ b_i \ne b_k}}^{m}\sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^{2} \psi(c) \cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
			&= \frac{1}{m^{n-2}} \sum_{\substack{c_\nu = 0\\ \nu \ne i,k}}^{2} \psi(c) \cdot \beta_{ijk}^{(1)}(c) \cdot \beta_{kli}^{(2)}(c)\\
		\end{aligned},$$ 
\end{abc}
where we have introduced the macro states $c_{\nu}.$ The state $c_\nu = 1$ represents the case $b_\nu = b_i$, the state $c_\nu = 2$ represents the case $b_\nu = b_k,$ and the state $c_\nu = 0$ representes any other case. Hence the weights for $c_\nu = 0, 1, 2$ are $m-2, 1, 1$ respectively which are gathered in the factor $\psi(c).$

\end{proof} 



\begin{cor}[Nakagami-m Fading, \cite{Nakagami12}]
	$$\E X_{ij} = \cdots $$
and
    $$\alpha_{i'j'k'}= \cdots$$
    $$\beta_{i'j'k'}= \cdots$$
	
	
	\comment{Currently, only the part where sending and receiving is allowed (so the prefactor of the ICCCN formula is missing in this result)}
\end{cor}

\begin{rem}
For Nakagami-Parameter=1 (Rayleigh fading) we recover the probabilities of [ICCCN19] for the full duplex case, i.e. ignoring the prefactor.   
\end{rem}
\begin{proof}
	$$\begin{aligned} \E X_{ij} = \E X_{ij}^{S_i} &= P(\frac{P_{ij}}{N+\sum_{l\ne i,j}\delta_{S_l S_i} P_{l j}} \ge \theta)\\
		&= \E \prod_{l\ne i,j}\exp\left\{ -\mu_{i j} \theta(N+ \delta_{S_i S_l} P_{l j})  \right\}\\
		&= \prod_{l\ne i,j} \E \exp\left\{ -\mu_{i j} \theta(N+ \delta_{S_i S_l} P_{l j})  \right\}\\
		&= \frac{1}{m^2} e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \sum_{\nu,\mu = 1}^{m}\E \exp\left\{ -\mu_{\nu j } \theta \delta_{\nu \mu} P_{l j} \right\}\\
		&= \frac{1}{m^2} e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( (m^2 - m) + \sum_{\nu=1}^{m} \E e^{-\mu_{i j}\theta P_{lj}} \right)\\
		&=  e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( (1-\frac{1}{m}) + \frac{1}{m}\cdot\frac{1}{1+\theta \frac{\mu_{i j}}{\mu_{lj}}} \right)\\
		&=  e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( 1 - \frac{1}{m}\cdot \frac{\theta \frac{\mu_{i j}}{\mu_{lj}}}{\theta \frac{\mu_{i j}}{\mu_{lj}} +1} \right)\\
		&=  e^{-\mu_{i j} \theta N } \prod_{l\ne i,j} \left( 1 - \frac{1}{m} \cdot \frac{\theta}{\theta + \frac{\mu_{lj}}{ \mu_{i j} }} \right)
	\end{aligned}$$
 \end{proof}



